Exploring the Geometry and Topology of Neural Network Loss Landscapes

Recent work has established clear links between the generalization performance of trained neural networks and the geometry of their loss landscape near the local minima to which they converge. This suggests that qualitative and quantitative examination of the loss landscape geometry could yield insights about neural network generalization performance during training. To this end, researchers have proposed visualizing the loss landscape through the use of simple dimensionality reduction techniques. However, such visualization methods have been limited by their linear nature and only capture features in one or two dimensions, thus restricting sampling of the loss landscape to lines or planes. Here, we expand and improve upon these in three ways. First, we present a novel "jump and retrain" procedure for sampling relevant portions of the loss landscape. We show that the resulting sampled data holds more meaningful information about the network's ability to generalize. Next, we show that non-linear dimensionality reduction of the jump and retrain trajectories via PHATE, a trajectory and manifold-preserving method, allows us to visualize differences between networks that are generalizing well vs poorly. Finally, we combine PHATE trajectories with a computational homology characterization to quantify trajectory differences.

==> neurips2021_files/neurips_paper_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}{}
\end{enumerate}

\item If you are including theoretical results... \answerNo{}
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} {\bf see Section \ref{ss:experimental_setup}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} {\bf see Appendix \ref{a:robustness_hi_res}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} {\bf see Section \ref{ss:experimental_setup}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} {\bf see Section \ref{ss:experimental_setup} and also done throughout the paper}
  \item Did you mention the license of the assets?
    \answerYes{} {\bf see Section \ref{ss:experimental_setup}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} {\bf all data used was open-source}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects... \answerNo{}
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> neurips2021_files/sections_neurips_clean/1_abstract.tex <==
\begin{abstract}
Recent work has established clear links between the generalization performance of trained neural networks and the geometry of their loss landscape near the local minima to which they converge. This suggests that qualitative and quantitative examination of the loss landscape geometry could yield insights about neural network generalization performance during training. To this end, researchers have proposed visualizing the loss landscape through the use of simple dimensionality reduction techniques. However, such visualization methods have been limited by their linear nature and only capture features in one or two dimensions, thus restricting sampling of the loss landscape to lines or planes. Here, we expand and improve upon these in three ways. First, we present a novel ``jump and retrain'' procedure for sampling relevant portions of the loss landscape. We show that the resulting sampled data holds more meaningful information about the network's ability to generalize. Next, we show that non-linear dimensionality reduction of the jump and retrain trajectories via PHATE, a trajectory and manifold-preserving method, allows us to visualize differences between networks that are generalizing well vs poorly. Finally, we combine the PHATE trajectories with a computational homology characterization to quantify the differences in trajectories.

\keywords{Artificial neural network loss landscape  \and Non-linear dimensionality reduction \and Topological data analysis.}
\end{abstract}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commented text from the NeurIPS submission
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% showed how simple dimensionality reduction and visualization techniques can be applied to this problem. However, so far such efforts have had limited success due to the limited sampling approaches and simple linear visualization techniques.

% After Guillaume's comments
% Recent work has established clear links between a deep network's loss landscape geometry near local minima, and the associated generalization performance. This suggests that qualitative and quantitative examination of a loss landscape's geometry could yield insights about neural network generalization performance during training. To this end, recent work showed how simple dimensionality reduction and visualization techniques can be applied to this problem. However, so far such efforts have had limited success due to the limited sampling approaches and simple linear visualization techniques. Here, we expand and improve upon these in three ways. First, we present a novel ``jump and retrain'' procedure for sampling relevant portions of the loss landscape. We show that the resulting sampled data holds more meaningful information about the network's ability to generalize. Next, we show that non-linear dimensionality reduction of the jump and retrain trajectories via PHATE, a trajectory and manifold-preserving method, allows us to visualize differences between networks that are generalizing well vs poorly. Finally, we combine the PHATE trajectories with computational homology characterization to quantify the differences in trajectories. 

% May 20 10pm version (After Smita's rewriting?)
% The training of deep neural networks involves traversal of a loss landscape that is determined by the network architecture, training data, and optimization loss terms. Specific training procedures (i.e.,  variants of stochastic gradient descent) lead to network convergence to local minima. Researchers have shown that the quality of such minima in large part determines the generalizability of the trained network to test data, as opposed to an overfitting of the training data. This leads to the hypothesis that qualitative and quantitative examination of the loss landscape could yield insights about neural network learning during training. To this end, past work has proposed visualization of loss landscape in low dimensions.  However, past visualization methods have been limited by their linear nature and only capture features in one or two dimensions, thus restricting sampling of the loss landscape to lines or planes. Here, we expand and improve upon these in three ways. First, we present a novel ``jump and retrain'' procedure for sampling relevant portions of the loss landscape. We show that the resulting sampled data holds more meaningful information about the network's ability to generalize. Next, we show that non-linear dimensionality reduction of the jump and retrain trajectories via PHATE, a trajectory and manifold-preserving method, allows us to visualize differences between networks that are generalizing well vs poorly. Finally, we combine the PHATE trajectories with computational homology characterization to quantify the differences in trajectories. 

% May 21st, 12h version (Stefan and Jessie)
%Training artificial neural networks requires the optimization of highly non-convex loss functions. Researchers have developed an extensive set of tools and architectures  that render this optimization task tractable. Despite this, the difference in trainability in between architectures, tasks and even the gap in network generalization capabilities still remain for the most part unexplained. Visualization tools combined with simple yet effective sampling procedures have played a key role in uncovering key geometric characteristics of the loss-landscape of ANNs and how they impact trainability and generalization capabilities.  However, past visualization methods have been limited by their linear nature and only capture features in one or two dimensions, thus restricting sampling of the loss landscape to lines or planes. We present a novel way of dynamically sampling the loss landscape surrounding a found optima {by following a ``jump and retrain'' procedure} and show that the resulting sampled data holds more meaningful information about the network's ability to generalize. The application of the modern dimensionality reduction method PHATE allows us to capture both global and local structures from the high-dimensional sampled data. The resulting visualizations reveal differences in generalization capabilities if used to make comparisons between initializations, architectures, and datasets. Finally combining PHATE with topological data analysis allows us to quantitatively compare the geometry of the sampled regions in the parameter space. Given these successes we anticipate that our sampling procedure, visualization method and TDA quantifications can be used in making informed choices about these aspects of neural networks.

%
%
% In an effort to uncover the difference in loss-landscape of ANNs in between architectures, tasks and their impact on network generalization capabilities, visualization tools combined with simple yet effective sampling procedures have been used.
%
% However, loss landscape sampling procedures have mainly consisted of sampling points from lines or planes in parameter space and most visualization methods have been relatively limited due to their linear nature and only capture features in one or two dimensions.
% Throughout the years, the scientific community has developed an extensive set of tools and architectures that render this optimization task tractable and a general intuition has been developed for choosing hyper parameters that help the models reach minima that generalize well to unseen data% and a general intuition has been developed for choosing hyper parameters that help the models reach minima that generalize well to unseen data. 
% and training hyper parameters than the sampling method commonly used in the literature. 
% reveals differences in generalization capabilities if used to make comparisons between initializations, architectures, and datasets.
% We also propose the use of the modern dimensionality reduction method PHATE to visualize the loss landscape since it represents the SOTA in terms of capturing both global and local structures of high-dimensional data. When applied to the data generated by our sampling procedure, this visualization method reveals differences in generalization capabilities if used to make comparisons between initializations, architectures, and datasets. %
% Finally we use topological data analysis to build an analysis pipeline based on a loss-level filtration of the sampled points which allows to extract meaningful topological characteristics of the loss landscape of ANNs which we then link to the model's performance, architecture and training procedure.

==> neurips2021_files/sections_neurips_clean/2_introduction.tex <==
\section{Introduction}
\vspace{-7pt}
Artificial neural networks (ANNs) have been successfully used to solve a number of complex tasks in a diverse array of domains, such as object recognition, machine translation, image generation, 3D protein structure prediction and many more. Despite being highly overparameterized for the tasks they solve, and having the capacity to memorize the entire training data, ANNs tend to generalize to unseen data. This is a spectacular feat since their highly non-convex optimization landscape should (theoretically) be a significant obstacle to using these models \cite{np_complete}. Questions such as why ANNs favor generalization over memorization and why they find ``good" minima even with intricate loss functions still remain largely unanswered. One promising research direction for answering them is to study the geometry of the loss-landscape of deep learning models. Recent work tried to approach this task by proposing various sampling procedures and visualization methods. An emerging challenge here is how to sample and look at such an extremely high dimensional optimization landscape (linear in the number of parameters of the network) with respect to minimized loss. 

In past work, loss functions and their level curves were visualized in random directions starting at a minimum, or by means of linear methods like PCA. In some cases, this approach proved effective in uncovering underlying structures in the loss-landscape and linking them to network characteristics, such as generalization capabilities or structural features \cite{goodfellow2014qualitatively,keskar2016large_batch,im2016empirical_loss_surfaces,Goldstein_LL_NIPS2018_7875}. However, these methods have two major drawbacks: \textbf{(1)} they are linear in that they only choose directions that are linear combinations of parameter axes while the loss landscape itself is highly nonlinear, and \textbf{(2)} they choose only one or two among thousands (if not millions) of axes to sample and visualize and ignore all others. 
% We review past work in Appendix \ref{s:related_work}. 

First, any dimensionality reduction algorithm would face difficulty in visualizing the loss landscape over the high-dimensional parameter space of ANNs, or even the entire training region that a neural network can cover. Instead, we posit that one can utilize a manifold structure inherent to relevant connected patches of the loss landscape that are reachable during training processes in order to faithfully visualize the essential characteristics of its ``shape'' and reflect on the insights they provide on the properties of the trained networks. For this, we propose a {\em jump and retrain} sampling method for the loss landscape that involves starting from a converged minimum and then perturbing and retraining the network from the perturbation. We show that this sampling method captures trajectories around the found minimum in a way that preserves information pertaining to the generalization capability of the neural network, while maintaining tractability of the visualization. 
% We show that this sampling strategy preserves generalization information by showing that a classifier can be trained from this data that actually predicts neural network test error with greater accuracy. 

We then utilize and adapt the PHATE dimensionality reduction method~\cite{phate}, which relies on diffusion-based manifold learning, to visualize these trajectories in low dimensions. In general, visualizations like PHATE are specifically designed to retain and compress as much variability as possible into two dimensions, and thus provide an advantage over previous approaches such as PCA. Our choice of using PHATE over other popular methods, such as tSNE~\cite{tsne}, is due to its ability to capture global and local structures of data, and in particular to keep intact the training trajectories that are traversed during gradient descent. We show that PHATE is suitable to track such continuous weight trajectories, as opposed to tSNE or UMAP \cite{umap} that tend to shatter them, and thus allows for significantly better visualizations of the manifolds on which these trajectories lie. 

Finally, we turn to topological data analysis (TDA) methods to quantify features of the jump and retrain trajectories,  and thus characterize the loss-landscape regions surrounding different optima that emerge in networks that generalize well vs poorly. Our approach provides a general view of relevant geometric and topological patterns that emerge in the high-dimensional parameter space, providing insights regarding the properties of ANN training and reflecting on their impact on the loss landscape. 

\vspace{-5pt}
\paragraph{Contributions:}
We present the jump and retrain sampling procedure in Section \ref{ss:methods_sampling} and show that the resulting data holds more relevant information about network generalization capabilities than past sampling procedures in Section \ref{ss:results_sampling}. We propose a new loss-landscape visualization method based on a variation of PHATE, implemented with cosine distance in Section \ref{ss:feature extraction}. Our visualization method is, to our knowledge, different from all other proposed methods for loss-landscape visualization in that it is naturally nonlinear and captures data characteristics from all dimensions. In Section \ref{ss:results_visualization}, we show that our method uncovers key geometric patterns characterizing loss-landscape regions surrounding good and bad generalization optima, as well as memorization optima. Finally, we use topological data analysis to characterize the PHATE transformed sampled manifolds and to quantify the differences between them in Section \ref{ss:results_tda}. To our knowledge this is the first time that a combination of data geometry (via PHATE) and topology has been used to analyze the loss landscape of ANNs.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commented text from the NeurIPS submission
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In this work we propose a novel loss-landscape sampling procedure aimed at dynamically sampling the low-loss manifolds visited by neural network optimizers during training. Indeed, during training, the high-dimensional neural networks weights change significantly while remaining on a connected manifold defined by the support of viable configurations (e.g., with sufficiently low training loss), which we refer to when discussing the geometry of the loss landscape.

% Previous version
% In this work we utilize and adapt the PHATE dimensionality reduction method~\citep{phate}, which relies on diffusion-based manifold learning, to study ANN loss landscapes by visualizing the evolution of network weights during training in low dimensions. In general, visualizations like PHATE~\cite{phate} are specifically designed to squeeze as much variability as possible into two dimensions, and thus provide an advantage over previous approaches. In particular our choice of using PHATE over other popular methods, such as tSNE~\citep{tsne}, is due to its ability to capture global and local structures of data, and in particular to keep intact the training trajectories that are traversed through during gradient descent. Indeed, during training, the high-dimensional neural networks weights change significantly while remaining on a connected manifold defined by the support of viable configurations (e.g., with sufficiently low training loss), which we refer to when discussing the geometry of the loss landscape. Inspired by this geometrical intuition we also present a novel loss landscape sampling procedure aimed at dynamically finding points situated on these connected manifolds through training. We show that PHATE is suitable to track such continuous weight trajectories, as opposed to tSNE or UMAP that tend to shatter them. Furthermore we use topological data analysis and a loss-level filtration to quantify the topological features of the found manifolds. We then link these topological features as well as the loss values sampled to the networks generalization capabilities, it's depth and width and the hyperparameters used during training, namely batch size, weight decay and data augmentation. Our approach provides general view of relevant geometric and topological patterns that emerge in the high-dimensional parameter space, providing insights regarding the properties of ANN training and reflecting on their impact on the loss landscape. 

%We propose a novel loss-landscape sampling procedure and a novel visualization method based on a variation of PHATE, implemented with cosine distance in Section \ref{s:methods}. Our visualization method is, to our knowledge, different from all other proposed methods for loss-landscape visualization in that it is naturally nonlinear and captures data characteristics from all dimensions. In Section \ref{ss:visualization}, we show that our method uncovers key geometric patterns characterizing loss-landscape regions surrounding good and bad generalization optima, as well as memorization optima. In Section \ref{s:methods} we also present a topological data analysis (TDA) pipeline that utilizes a loss-level filtration to extract the topological features of the manifolds reconstructed from the sampled data. Finally we show that the loss values sampled with our method and the topological features we computed hold meaningful information about the networks ability to generalize, it's depth, width and the hyperparameters used to find the optimum. To our knowledge this is the first time TDA is used to analyze the loss landscape of ANNs and the links between the geometrical and topological characteristics of the loss region surrounding the optimum and the training hyperparameters used to find the optimum are novel.

==> neurips2021_files/sections_neurips_clean/3_preliminaries.tex <==
\vspace{-5pt}
\section{Preliminaries}\label{s:preliminaries}
\vspace{-7pt}

\subsection{PHATE dimensionality reduction \& visualization}\label{ss:phate}
% Given an $n\times m$ data matrix $\mathbf{N}$, where $n$ is the number of data points and $m$ the number of features, 
Given a data set, PHATE computes low-dimensional embeddings of the data points %(dimension $d$ to be specified by the user)
which preserve both their global and their local structure. It first computes the pairwise distance matrix $\mathbf{D}$ using a specified distance function $\phi$
%, each element of the matrix being given by $\mathbf{D}_{ij}=\phi(\mathbf{N}_{i,:},\mathbf{N}_{j,:})$
. To better capture local affinities between data points, an affinity matrix $\mathbf{A}$ is computed using an $\alpha$-decaying kernel with a locally-adaptive bandwidth $\epsilon_{k,i}$ corresponding to the $k$-NN distance of the $i$-th data point. The elements of $\mathbf{A}$ are given by:
\[\mathbf{A}_{i,j}=K_{k,\alpha}(i,j)=\frac{1}{2}\exp\left(-\left(\frac{D_{i,j}}{\epsilon_{k,i}}\right)^\alpha\right)+\frac{1}{2}\exp\left(-\left(\frac{D_{i,j}}{\epsilon_{k,j}}\right)^\alpha\right)\]
The decaying factor $\alpha$ regulates the decay rate of the kernel (smaller $\alpha$ $\Rightarrow$ kernel with lighter tails), $\alpha = 2$ corresponding to the Gaussian. The affinity matrix is then row-normalized to obtain the diffusion operator $\mathbf{P}$, a row-stochastic Markov transition matrix with element $\mathbf{P}_{i,j}$ giving the probability of jumping from the $i$-th to the $j$-th data point in one time step. One of the reasons PHATE excels at capturing global structures in data, especially high-dimensional trajectories and branches, is that it leverages the diffusion operator (also used to construct diffusion maps]\cite{COIFMAN20065_Diffusion_Maps}) by running the implicit Markov chain forward in time. This is accomplished by raising the matrix $\mathbf{P}$ to the power $t$, effectively taking $t$ random walk steps and revealing intrinsic geometric structure through the affinity of the data at a scale that grows with the number of steps. The optimal value for $t$ is automatically chosen to be the knee point of the von Neumann entropy of $\mathbf{P}$. 

To enable dimensionality reduction while retaining diffusion geometry information from the operator, PHATE leverages information geometry to define a pairwise {\em potential distance} as an M-divergence $\mathbf{ID}_{i,j}=\|\log P_{i,:} - \log P_{j,:}\|_2$ between corresponding $t$-step diffusion probability distributions of the two points, which provides a {\em global context} to each data point. The resulting information distance matrix $\mathbf{ID}$ is finally embedded into a visualizable low dimensional (generally 2D or 3D) space by metric multidimensional scaling (MDS), thereby squeezing the intrinsic geometric information into two dimensions (as is also done in tSNE), rather than producing a high dimensional alternative coordinate system like PCA or diffusion maps.

We conjecture that since PHATE learns a data manifold via diffusion, and places points in the global context of other points, it can keep trajectories connected from beginning to end without shattering them. Indeed, this property was established quantitatively in~\cite{phate} via a Denoised Manifold Affinity Preservation (DeMAP) metric. Here, it leads to the preservation of trajectory flow directions and relations between them, as demonstrated in Figure \ref{fig:dim_red_comparison}, 
%in comparison with other methods, 
on trajectory-like data and ANN training trajectories, as well as in our results presented in the remainder of the paper.

\vspace{-5pt}
\subsection{Topological data analysis}\label{sec:Topological data analysis}
\vspace{-3pt}
Topological data analysis~(TDA) refers to a set of techniques for
understanding complex datasets by means of their topological features,
i.e., their connectivity~\cite{Edelsbrunner10}. While TDA is applicable
in multiple contexts, we focus specifically on the case of graphs. Here,
the simplest set of topological features is given by the number of
connected components~$\betti{0}$ and the number of cycles~$\betti{1}$,
respectively. Such counts, also known as the \emph{Betti numbers}, are
coarse graph descriptors that are invariant under graph isomorphisms.
Their expressivity is somewhat limited, but can be increased by
considering a function $f\colon V \to \reals$ on the vertices of a
graph~$G = (V, E)$ with vertex set~$V$ and edge set~$E$. Since $V$ has
finite cardinality, so does the image~$\im f$, i.e.,
$\im f := \{w_1, w_2, \dots, w_n \}$.
Without loss of generality, we assume that $w_1 \leq \dots \leq w_n$. We
write $G_i$ for the subgraph induced by filtering according to $w_i$,
such that the vertices of $G_i$ satisfy $V_i := \{ v \in V \mid f(v)
\leq w_i\}$, and the edges satisfy $E_i := \{ (u, v) \in E \mid
\max(f(u), f(v)) \leq w_i \}$. The subgraphs $G_i$ satisfy a nesting
property, as $G_1 \subseteq G_2 \subseteq \dots \subseteq G_n$. It is
now possible to calculate topological features alongside this
\emph{filtration} of graphs, tracking their appearance and
disappearance. If a topological feature is created in $G_i$, but
destroyed in $G_j$~(it might be destroyed because two connected
components merge, for instance), we represent this by storing the point
$(w_i, w_j)$ in the \emph{persistence diagram} $\mathcal{D}_f$ associated to $G$.

Persistence diagrams are known to be salient descriptors of graphs and
have seen increasing usage in graph classification~\cite{Hofer17,Hofer20,Rieck19b,Zhao19}. Their primary appeal lies in their
capability to summarize shape information and, through simple
coordinate transformations~\cite{Adams17,hofer2019learning}, being
amenable to the inclusion in standard machine learning pipelines.
Topological features are of particular appeal in case invariance to
certain geometric operations is desired; their robustness to
noise~\cite{Cohen-Steiner07} made them successful shape descriptors in
a variety of applications~\cite{Amezquita20,Rieck20}. Numerous fixed
filtrations have been described for different tasks~\cite{Hofer20,Zhao19}, but in our context, a natural choice for~$f$ is provided by the
\emph{loss function} of the network itself. This will enable us to describe
the topology of the loss landscape.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commented text from the NeurIPS submission
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In this section we explain how the method PHATE \citep{phate} works, and the theoretical reasons behind PHATE's success at capturing global trajectories structures in data.
% \vspace{-3pt}

==> neurips2021_files/sections_neurips_clean/4_methods.tex <==
\vspace{-5pt}
\section{What is the ``shape'' of the loss landscape?}\label{s:methods}
\vspace{-7pt}

The loss landscape of an ANN (or generally a parameterized model trained via loss minimization) can be formulated mathematically as the geometry and topology defined in the high dimensional parameter space $\Theta$ by a loss function $f\colon\Theta \to \mathbbm{R}$ that assigns a loss value $f(\theta)$ to every possible parameter vector $\theta$ (e.g., consisting of network weights) based on considered training or validation data. While $f(\theta)$ provides some information for examining and filtering the various configurations of model parameters, the exuberantly high dimensionality of the parameter space (i.e., often in the millions) renders the task of visualizing or analyzing the entire loss-landscape over $\Theta$ virtually impossible. However, since the optimization process considered in this context is guided by the objective of minimizing the loss, we can expect most regions in the high dimensional $\Theta$ to be of negligible importance, if not unreachable, for the network training dynamics or the viable configurations learned by them. Therefore, the analysis of the loss landscape can focus on regions that are reachable, or reliably traversed, during this optimization process, which we expect would have a much lower intrinsic dimensionality than the ambient dimensions of the entire parameter space. 

Our approach to characterizing the ``shape'' of the loss landscape in such local regions of interest is inspired by the construction of a tangent space of manifolds in intrinsic terms in Riemannian geometry. There, tangent vectors at a given point of interest are defined by aggregating together intrinsic trajectories (on the manifold) traversing through the tangential point. This aggregation, in turn, yields equivalence classes that signify tangential directions, whose span is considered as the tangent space that provides a local intrinsic (typically low dimensional) coordinate neighborhood in the vicinity of the tangential point. In a similar way, here we proposed to leverage trajectories of the network optimization process in order to reveal the intrinsic geometry exposed by them as they flow towards convergence to (local) minima of the loss. The remainder of this section provides detailed derivation of the three main steps in our approach. First, the sampling of trajectories in significant regions of the loss landscape (i.e., near local minima), then their aggregation into a visualization and representation capturing local geometry, and finally the extraction of topological descriptors providing quantitative characterization of the ``shape'' of the examined loss landscape regions.

\vspace{-5pt}
\subsection{Jump and retrain sampling}\label{ss:methods_sampling}
\vspace{-5pt}
Gradient based optimization methods naturally explore low-loss regions in parameter space before finding and settling at a minimum. We hypothesize that keeping track of optimizer trajectories in parameter space is an efficient way of sampling these low-loss manifolds and thus to gather information about the relevant part of the loss regions surrounding minima. This can be seen as an approximation to the Morse--Smale complex~\cite{Gyulassy08}, a decomposition of~$f$ into regions of similar gradient behavior, whose analytical calculation is infeasible given the overall size of $\Theta$. With this in mind we have designed the following ``jump and retrain'' or J\&R sampling procedure. Most of our experiments were conducted with \texttt{SEEDS}$=\{0,1,2,3\}$ or $\{0,1,2,3,4\}$, \texttt{STEP\_SIZES}$=\{0.25, 0.5, 0.75, 1.0\}$ and $N=40$ or $50$.

\begin{itemize}[nosep, leftmargin=*]
    \item Let $\theta_o$ represent the vector of network parameters at the minimum;
    \item For $seed\in$ \texttt{SEEDS}:%\{0,1,2,3\}$:
    \begin{itemize}[nosep]
        \item For $step\_size\in$ \texttt{STEP\_SIZES}: % \{0.25, 0.5, 0.75, 1\}$:
        \begin{enumerate}[nosep]
            \item Choose a random $v_{seed}$ in  $\Theta$ given the random seed and filter-normalize to obtain $\overline{v}_{seed}$;
            \item Set the ANN parameters at each jump initialization to be $\theta_{\text{jump-init}} = \theta_o + step\_size \cdot \overline{v}_{seed}$;
            \item Retrain for $N$ epochs with the original optimizer; % on the ``retraining'' data set;
            \item Record network parameters $\theta$ and evaluate the loss at each epoch during retraining;
        \end{enumerate}
    \end{itemize}
\end{itemize}

% Assuming the full training data set was used to reach $\theta_o$ (the base optimization minimum), this data set can then be split into what we name the retraining data set (90\% of the original one) and the validation data set (remaining 10\% of data points). All examples from both these data sets have been used when originally training the network but the examples from the validation data set will not be seen by the model throughout the retraining procedure. Most of our experiments were conducted with \texttt{SEEDS}$=\{0,1,2,3\}$ or $\{0,1,2,3,4\}$, \texttt{STEP\_SIZES}$=\{0.25, 0.5, 0.75, 1.0\}$ and $N=40$ or $50$.

\vspace{-7pt}
\subsection{PHATE dimensionality reduction and visualization}\label{ss:feature extraction}
\vspace{-7pt}
Since the points sampled with the presented procedure are not simply positioned on a line or a plane, methods that project these points onto a 1D or 2D space are unable to properly visualize all the variation in the data.
%
PHATE has allowed us to bypass the key drawbacks of previously proposed linear interpolation visualization methods by \textbf{(1)} Capturing variance in the sampled data from all relevant dimensions and embed it in a low-dimensional space; and \textbf{(2)} preserving high-dimensional trajectories and global structures of data in parameter space. All modern dimensionality-reduction techniques would have achieved \textbf{(1)} in one way or another with varying degrees of success. However our proposed cosine-distance PHATE has unique advantages over other state-of the art dimensionality reduction methods to accomplish \textbf{(2)}. Figure~\ref{fig:dim_red_comparison} demonstrates this by showing a comparison of multiple such techniques, namely PHATE, PCA, t-SNE \cite{tsne} and UMAP \cite{umap}, and how they each embed the data from the J\&R sampling (Fig. \ref{fig:dim_red_comparison}\textbf{A} and \textbf{B})  and an artificial data set having a tree-like structure (Fig. \ref{fig:dim_red_comparison}\textbf{C}) in a 2D space.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/comp_fig.png}
    \caption{2D embeddings of the J\&R experiment (5 random seeds) results for a WResNet28-2 network using PHATE (\textbf{1}), t-SNE (\textbf{2}), UMAP (\textbf{3}) with euclidean (\textbf{A}) and cosine (\textbf{B}) distances and the linear methods PCA (\textbf{A4}) and random plane projection (\textbf{B4}). \textbf{C:} embeddings found using the same techniques of an artificial data set having a fully connected tree-like structure. We see that PHATE consistently retains continuous trajectory structures while other embeddings (tSNE/UMAP) shatter the structure, or show chaotic trends (PCA, random directions) because of uninformative projections to low dimensions.
    % See Appendix \ref{a:dim_red_comparison_hi_res} for higher resolution.
    }
    \label{fig:dim_red_comparison}
    \vspace{-5pt}
\end{figure}

While some trajectory-like structure is visible in all low-dimensional embeddings, only PHATE properly captures intra-trajectory variance. PHATE is also the only technique that captures the global relationships between trajectories while t-SNE and UMAP have a tendency to cluster points that are close in parameter space and disregard the global structure of the data. On the artificial data set (Fig. \ref{fig:dim_red_comparison} \textbf{C}), what we observe is that the embeddings of the linear method PCA are highly affected by the noise in the data while t-SNE and UMAP have a tendency of shattering trajectories that should be connected.  By accomplishing \textbf{(1)} and \textbf{(2)} PHATE effectively reconstructs the manifold in parameter space from which the jump and retrain data is sampled and allows it's embedding in a lower dimensional space preserving its local and global structure.

\vspace{-5pt}
\subsection{Topological feature extraction}\label{ss:quantifying}
\vspace{-5pt}
In order to quantify the shape of the PHATE embeddings, we calculate a set of topological features. To this end, we first compute a kNN graph~(with $k = 20$) based on the PHATE diffusion potential distance. Each node of this graph~$G$ corresponds to a specific point~$\theta \in \Theta$ sampled from the loss landscape. We obtain a filtration function from this by assigning each vertex $\theta$, which corresponds to a setting of the parameters of the neural network its corresponding loss value $f(\theta)$. Then we filter over this graph by slowly increasing the loss threshold $t$, which effectively reveals larger and larger parts of the graph and creates a homology as described in Section~\ref{sec:Topological data analysis}. From this homology we obtain a set of persistence diagrams $\mathcal{D}_0$, $\mathcal{D}_1$ summarizing the topological features of the respective embedding~(we omit the index~$f$ for simplicity). We note that this filtration is not the commonly used Vietoris-Rips filtration which is based on a distance threshold between points. 
%
As a powerful summary statistic, we calculate the \emph{total persistence}~\cite{Cohen-Steiner07} of a persistence diagram~$\mathcal{D}$, i.e.,
%
$\operatorname{pers}(\mathcal{D}) := \sum_{(c, d) \in \mathcal{D}} \left|d - c\right|^2$. $\operatorname{pers}(\cdot)$ serves as a complexity measure that enables us to compare different embeddings. This measure has the advantage that it is invariant with respect to rotations of the embedding. Moreover, it satisfies robustness properties, meaning that it will change continuously under a continuous perturbation of the input filtration. If two loss functions~$f$ and~$f'$ are \emph{close}~(in the Hausdorff sense), their corresponding total persistence values will be close as well, making this value a useful summary statistic.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commented text from the NeurIPS submission
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% When trying to design a novel loss-landscape sampling procedure it is natural to think about the process of training. In general, the vast parameter space of deep learning models is mostly unexplored except for a few points that lie on the optimizer path between initialization and optimum. However, it is these training trajectories that determine the ultimate performance of our model. By gathering locally connected loss-landscape patches throughout training, we can hope to reconstruct manifolds on which these trajectories lie. Despite the thousands, if not millions, of dimensions of the parameter space, we hypothesize that these trajectories and manifolds are intrinsically of low dimension and thus PHATE, which reduced dimensionality via manifold learning and information geometry, will help facilitate their visualization and the analysis of their characteristics. With this in mind we have designed the following ``jump and retrain'' or J\&R sampling procedure:

% In order to compare the results of this sampling procedure across networks it is important that the optimizer and hyperparameters used during retraining are identical across networks independently of the original training procedure with which the initial optimum $\theta_o$ was reached.

% As a general note the networks seem to achieve almost 100\% accuracy on the retraining data set as expected and tend to perform significantly better (although not 100\%) on the validation data set than on the test data set. We explain this by the fact that the jump and retraining sampling procedure samples the region of the loss landscape surrounding a minima that was found during training which used the validation data set. Even if the jump changes the parameters some information still remains.

% The spaces and planes change as retraining progresses. It is thus more appropriate to use all dimensions of the parameter space instead of linear projection methods such as PCA. 


% While the PHATE embeddings are perfect for visualization purposes since information from all directions of variation in the data is squeezed into two dimensions, visualizations can sometimes be hard to interpret and are inherently hard to use at scale since they require human input to conduct comparisons. For a more advanced analysis it is hence necessary to derive a quantification of the relevant loss landscape characteristics. Our quantification method uses the PHATE diffusion potentials from which the embeddings are computed and which holds all relevant information about both the local and the global structure of the data. As previously mentioned this information can be seen as the reconstruction of the manifold from which the points were sampled, the goal here is to quantify the structure of this manifold by computing it's topological features via topological data analysis. We also compare the topological features derived from the PHATE diffusion operator to the topological features derived from the distance matrix between all points.

% In order to compute the topological features of the considered manifold we utilize the following procedure. First we compute the kNN adjacency matrix by using the PHATE diffusion potentials to find the nearest neighbors. 


% Previous beginning of the section
%We consider the following three sampling procedures designed to explore the loss-landscape region surrounding a given optimum $\theta_o \in \Theta$ found through typical ANN training. 
% The first procedure is inspired by the literature the two others are designed by us, all of them sample 640 points from the loss landscape excluding the optimum itself. While the number of points sampled is somewhat arbitrary, it is important to compare the methods with the same number of points. We found 640 points to hold enough information about the loss landscape while still being small enough for our experiments to run without any major computational challenges. Because of the effectiveness of the filter-wise normalization presented in \cite{Goldstein_LL_NIPS2018_7875}, we normalize all random vectors in parameter space in this manner.

% \paragraph{Grid sampling} 
% Similar to the 1D or 2D linear interpolation used in past visualization methods, we randomly choose 3 vectors starting from $\theta_o$ and construct a 3D grid using the 3 vectors as basis. The loss and accuracy on the training set is then evaluated at all points on the grid. 
% As discussed in the Related Work section, most loss landscape visualization methods are based on 1D or 2D linear interpolations. The loss landscape is in that case sampled by evaluating the loss at equally spaced points from a line or a plane in parameter space, all other dimensions are ignored. We adapt the grid sampling procedure to three dimensions. Three random directions are chosen in parameter space, $\theta_1, \theta_2, \theta_3$, because of the dimensionality of the space these directions are nearly orthogonal with high probability. The loss and accuracy on the training set is evaluated at points in parameter space corresponding to the sum of the parameters at the optimum and linear combinations of these directions, i.e. $\theta_o + c_1\theta_1 + c_2\theta_2 + c_3\theta_3$ with coefficients $c_1\in\{-1.0, -0.8, -0.6, -0.4, -0.2, 0.2, 0.4, 0.6 ,0.8, 1.0\}$ and $c_2, c_3 \in\{-0.8, -0.6, -0.4, -0.2, 0.2, 0.4, 0.6 ,0.8\}$.
% %
% %Certain geometrically inspired methods to evaluate the sharpness of a found minimum rely on computing the Hessian to determine the principal curvatures of the loss landscape at the minimum. However such methods are so computationally expensive that they are often conducted just at the optimum.

% \paragraph{Naive sampling} The grid structure of the previous sampling procedure makes it easy to construct interpretable plots of the loss landscape for visualization purposes. However, to our knowledge there is no prior result stating that such a rigid sampling of the loss landscape holds the most information about the landscape. We hypothesize that there are more efficient ways to sample the loss landscape in a way that is evocative of the network's ability to generalize. We propose the idea that using more directions and step sizes when sampling, without the grid-like structure, could be more informative since it explores a greater number of directions in parameter space. The naive sampling procedure selects 32 random vectors in parameter space, $\theta_i, i\in\{1,\ldots,32\}$, and evaluates the loss and accuracy on the training set at points corresponding to the sum of the parameters at the optimum and one of these directions multiplied by a step size. In other words we evaluate the loss and accuracy at the points $\theta_o + c\theta_i$ for $c\in\{0.05, 0.1, 0.15, \ldots, 0.95, 1.0\}$ (20 possible values) and $i\in\{1,\ldots, 32\}$.

% \paragraph{Jump and retrain sampling}
% While the two first sampling procedures are very easy to implement and sample the loss in an orderly manner, the information gathered about the loss is not used during the procedure itself. 

==> neurips2021_files/sections_neurips_clean/5_results.tex <==
\vspace{-5pt}
\section{Geometric and topological reflection on ANN training and generalization}\label{s:results}
\vspace{-7pt}
\subsection{Experimental setup}\label{ss:experimental_setup}
\vspace{-5pt}
In order to assess the effectiveness of our loss landscape visualizations and characterizations, we trained wide ResNets \cite{wide_resnet} of varied sizes with depth $\in \{10, 16, 22\}$, width $\in\{1,2\}$ on the CIFAR10 image classification task \cite{cifar10} from initialization to optimum. The networks were trained with a combination of the following hyperparameters: batch size $\in\{32, 128, 512\}$, weight decay $\in\{0, 0.0001, 0.001\}$ and either with or without data augmentation (random horizontal flips and crops). Each of the 108 WResNets were initialized identically and trained for 200 epochs using SGD with 0.9 momentum and a learning rate with initial value of 0.1 followed by step decay by a factor of 10 at epochs 100, 150 and 185.

We also trained WResNet28-2 networks on CIFAR10 using batches of size 128 for 200 epochs with the same optimizer, with combinations of data augmentation and weight decay. Utilizing data augmentation and weight decay has allowed us to find optima that generalize better, increasing test accuracy from around \textasciitilde85\% to \textasciitilde95\%. We will be referring the optima with \textasciitilde95\% test accuracy as ``good optima'' since they generalize better, and the others as ``bad optima''. Using the same training procedure as the one for the bad optima, we also trained a WResNet28-2 network for memorization by completely randomizing the labels of the training data. This modification was used in \cite{Zhang2017UnderstandingDL,closer_look_memorization,dnns_don't_learn_via_mem} to show that neural networks have the ability to completely memorize the training data sets.

Code made available online through the MIT license by the authors of \cite{Goldstein_LL_NIPS2018_7875} and \cite{Zhang2017UnderstandingDL} was adapted and used to run these experiments. The following open-source Python libraries were used: PyTorch \cite{NEURIPS2019_9015_pytorch}, Scikit-learn \cite{scikit-learn} and Giotto-tda \cite{tauzin2020giottotda}. The networks were trained using a Nvidia Titan RTX GPU.



\vspace{-5pt}
\subsection{Jump and retrain sampling captures generalization and training characteristics}\label{ss:results_sampling}
\vspace{-5pt}

\begin{table}[b]
\centering
\vspace{-20pt}
\caption{Mean and standard error (\%) of the 11 classifiers accuracies on the 5 class generalization, weight decay and data aug. classification tasks with different features.}
\label{tab:sampling_classif}
 \begin{tabular}{|M{7cm}|M{1.5cm}|M{1.5cm}|M{1.5cm}|}
 \hline
 Features & 5 class gen. & Weight decay & Data augmentation \\
 \hline
 Theoretical random (1/\#classes) & 20.0 & 33.3 & 50.0\\
 \hline
%  Randomized J\&R retrain loss and accuracy values & 20.7 $\pm$ 1.1 \\
 Randomized J\&R retrain loss and accuracy values & 20.7 $\pm$ 1.1 & 38.9 $\pm$ 1.5 & 52.7 $\pm$ 1.9 \\
 \hline \hline
 Grid sampling,  train loss and accuracy values & 30.1 $\pm$ 2.7 & 51.1 $\pm$ 2.9 & 62.3 $\pm$ 5.1 \\  
 \hline
 Naive sampling, train loss and accuracy values & 31.8 $\pm$ 4.0  & 55.7 $\pm$ 3.9 & 67.6 $\pm$ 5.2  \\
 \hline
 J\&R sampling, retrain loss and accuracy values & \textbf{39.2} $\pm$4.3  & \textbf{58.2} $\pm$3.6 &  \textbf{72.1} $\pm$5.4 \\
%  \hline
%  J\&R sampling, valid loss and accuracy values & 39.0 $\pm$ 4.1  \\
 \hline
\end{tabular}
\end{table}

%As discussed in Section \ref{s:related_work}, 
Past work has shown that networks with different generalization capabilities tend to have optima surrounded by regions of distinct geometrical characteristics \cite{Hochreiter1997_flat_minima,im2016empirical_loss_surfaces,Goldstein_LL_NIPS2018_7875,keskar2016large_batch,entropy_sgd}. Regularization techniques, such as weight decay and data augmentation, are believed to play a role in this difference in geometries \cite{entropy_sgd,im2016empirical_loss_surfaces}. Inspired by past results, we formulate the following classification tasks to evaluate loss landscape sampling methods and see if the sampled data holds information about the networks ability to generalize
%to unseen data
and the geometry of the loss landscape. We used the sampled loss and accuracy values as features and we separated the trained WResNet models into 5 (almost) equally-sized ``generalization'' classes according to the value of the test loss at optimum. The \textasciitilde20\% of networks with the lowest test losses at optimum were assigned to class 1, and so on. We then trained 11 simple classifiers 
%(see Appendix \ref{a:classifiers} 
for details) to predict the generalization class of each network with training losses and accuracy features. All results were obtained from  10-fold cross validation. It is important to note that the classifiers were not tuned to  favor any of the sampling procedures. Two similar classification tasks were designed to predict weight decay and whether or not data augmentation was used.

To evaluate the effectiveness of the jump and retrain sampling, we compared it to
%the results to those obtained with 
two other sampling procedures. We refer to the first as {\it grid sampling}, and it is directly inspired by the 1D or 2D linear interpolations used in past visualization methods \cite{goodfellow2014qualitatively,im2016empirical_loss_surfaces,Goldstein_LL_NIPS2018_7875}. Here, we randomly choose 3 vectors starting from the optimum ($\theta_o$) and construct a 3D grid using the 3 vectors as basis. The loss and accuracy on the training set is then evaluated at all points on the grid. The second comparison sampling procedure, that we call {\it naive sampling}, evaluates the loss in random directions ($\theta_i$) centered at the optimum $\theta_0$, and multiple step sizes $c$; i.e. evaluate at $\theta_o + c\theta_i$. This method tests whether using more directions and step sizes when sampling, without the grid-like structure, is more informative since it explores a greater number of directions in parameter space. All methods considered, including J\&R, sample 640 points from the loss landscape excluding the optimum itself. %While the number of points sampled is somewhat arbitrary, it is important to compare the methods with the same number of points. 
We found 640 points to hold enough information about the loss landscape while still being small enough for our experiments to run without any major computational challenges. We applied the filter-wise normalization presented in \cite{Goldstein_LL_NIPS2018_7875} when obtaining random directions. As a control experiment, we trained the same classifiers on scrambled versions of the best performing features, making sure classifiers were not overfitting the data and evaluating the impact of feature distributions alone. The mean and standard error across the 11 classifiers are shown in Table \ref{tab:sampling_classif}.

Using the loss and accuracy values sampled with the J\&R procedure as features allows the classifiers to achieve mean accuracies of 39.2\%, 58.2\% and 72.1\% on the generalization, weight decay and data augmentation classifications tasks respectively. This is significantly higher than the mean classification accuracies reached using the data sampled with the other two methods. We confirmed the validity of the classification accuracy with J\&R data with permutation tests where the accuracy is essentially the same as random. Indeed, our results indicate that connected patches of the low-loss manifold surrounding the optima, which are found with the jump and retrain procedure, hold more information about the region's geometry and the network's ability to generalize at that optimum than the data sampled with non-dynamical methods. Furthermore, the success of the J\&R sampled data on the weight decay and data augmentation classification tasks shows that our sampling method captures information not only about generalization but also about the training procedure. The set of J\&R sampled loss and accuracy values seem to have distinct characteristics depending on the training procedure used to reach the minima and whether or not regularization methods were used or not and to what extent. This helps support the idea that a dynamical sampling of the loss landscape, which mimics the behavior of standard optimization procedures, is more informative than static methods such as \textit{grid} or \textit{naive} sampling.

\vspace{-5pt}
\subsection{Generalization indicated by visual patterns from loss landscape regions around optima}\label{ss:results_visualization}
\vspace{-5pt}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/visualization_figure.png}
    \caption{\textbf{Top row:} PHATE embeddings of the data generated with the three sampling procedures colored by loss in log scale. The rigidity of the grid and naive sampling methods makes visualizations less informative.
    %since data sampled around different optima have similar low dimensional embeddings only with different values of loss at each point. 
    The J\&R sampling successfully samples the low-loss manifolds surrounding minima.
    \textbf{Bottom row:} PHATE embeddings comparison between good, bad and memorization minumum. The good and bad minimum models achieved 94.39\% and 87.29\% test accuracy at the end of J\&R experiments. The retraining initial points immediately after the jump are marked by diamonds of colors corresponding to $step\_size$ and trajectories are colored by their respective direction of the initial jump with descending hue, i.e. the color gets whiter as retraining progresses. In contrast to more continuous trajectories returning to near the optimum in the good generalization case, memorization displays a more random pattern where weights move out before moving back, often switching direction during retraining. Bad generalization appears to be more similar to memorization and without continuous trajectories.
    %The J\&R experiment (with 5 random seeds instead of 4) conducted and on one good and one bad generalization minima that achieve 94.39\% and 87.29\% accuracy on the test data respectively, as well as one memorization minimum. The initial points of the jumps (before retraining) are marked by diamonds of different colors based on $step\_size$ and  trajectories are colored by their respective direction of the initial jump with descending hue, i.e. the color gets whiter as retraining progresses. 
    }
    \label{fig:visualization}
    \vspace{-5pt}
\end{figure}

PHATE visualization of the data sampled with the J\&R procedure as in  Fig.~\ref{fig:visualization}(c) clearly demonstrate the trajectories and the low-loss manifold surrounding the found optima that was actually traversed during training. It is more informative that the visualization of data from the other two sampling procedures as in Fig~\ref{fig:visualization}(a) and (b). 


Although all networks achieved $\approx0$ loss on their respective training sets and only a \textasciitilde7\% difference in their accuracy on test sets, Fig.~\ref{fig:visualization}(d)-(f) reveal stark differences  between network configurations  that  memorize  (or  overfit)  versus  ones  that generalize. The minimum that shows good generalization has a distinctive star shaped pattern. This pattern indicates that even when points are thrown away from the minima they return to it immediately without traveling outward. Thus the minima seems to serve as an effective attractor to which trajectories repeatedly return.

In case of bad minimum, the trajectories start off near the middle of the plot (darker points in the middle of Fig.~\ref{fig:visualization}e) but during the retraining, the trajectories diverge toward the edges before occasionally coming back towards the middle of the plot. This outward movement is in stark contrast with the consistent retraining trajectories surrounding the good generalization minimum, which immediately return to the valley. Thus in this sense the minima are not stable and perturbations of the parameters cause networks to escape this minima.   The ``memorization'' minimum plot Fig.~\ref{fig:visualization}f) looks similar to the bad generalization plot, with trajectories that go outward at small step sizes of the jump. However, curiously at larger step sizes, the trajectories seem to return without going outward first,  but they do not return immediately, i.e., they show some lateral movement, potentially indicating bumpiness in the landscape that they are avoiding. 
%See supplemental video for an animation of these trajectories, and Appendix \ref{a:generalization_hi_res} for trajectories colored by loss.


%Shorter version of Robustness
One of the main problems encountered in previous attempts to visualize ANN loss landscapes resides in the difficulty of comparing them across tasks and initializations. We verified that our visualization method, applied to points sampled with the J\&R procedure, alleviates this concern by training multiple WResNet28-2 networks starting from different initializations and also on a different task (CIFAR 100). For all networks, regardless of initialization and the task they were trained on, the visualizations of the regions surrounding minima that generalize well show the same star shaped pattern which differ significantly from the ``bad'' optima visualizations.
% (see Appendix \ref{a:robustness_hi_res}).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/embeds_pers_diags_rect.png}
    \caption{\textbf{Top row:} 2D PHATE embeddings of the data sampled with the jump and retrain procedure surrounding minima reached by four WResNet16-2 with the same initialization but trained in different ways and thus reaching different accuracies on the test set. \textbf{Bottom row:} Persistence diagrams of the loss-level filtration computed from the respective PHATE diffusion potentials. The total persistence associated with each optima/persistence diagram is written in bold. Both PHATE and the topological features of the loss landscape seem to differentiate these four networks which have very different generalization capabilities.}
    \label{fig:tda_characterization}
    \vspace{-15pt}
\end{figure}

\vspace{-5pt}
\subsection{Generalization may be related to low topological activity in near-optimum regions}\label{ss:results_tda}
\vspace{-5pt}
PHATE has allowed us to generate low dimensional representations of the low-loss manifolds sampled through the jump and retrain procedure. Here, topological data analysis enables us to quantify the topological features of these manifolds and thus characterize the loss landscape regions surrounding different optima. In Fig.~\ref{fig:tda_characterization} we show the PHATE visualizations of the jump and retrain data sampled around different optima of a WResNet16-2 network and the corresponding dimension 0 and 1 persistence diagrams. From the PHATE visualizations alone it is clear that the sampled manifold have different structures. In fact, the persistence diagrams confirm that these manifolds also have different topological features. In particular, optima that generalize poorly seem be surrounded by manifolds with more topological activity, the two persistence diagrams on the left having more high-persistence points that are away from the diagonal (red rectangles in Fig. \ref{fig:tda_characterization}). This can be observed through the higher density of points in the upper left corner of the persistence diagrams. On the other hand networks that generalize well have both zero-dimensional and one dimensional topological features that emerge later in the loss threshold (to the right of the persistence diagrams in the green rectangles). 

\begin{wrapfigure}[14]{R}{0.4\textwidth}
    \vspace{-19pt}
    \includegraphics[width=\linewidth]{figures/pers_quant.png}
    \vspace{-22pt}
    \caption{Total persistence of dimension 0 computed from the jump \& retrain data for each network w.r.t.\ the test loss at optimum. Colors indicate the value of the weight decay used during training.}
    \label{fig:total_pers}
\end{wrapfigure}

In order to verify this observation in a more general case, we also computed the \emph{total persistence}~(see Section~\ref{ss:quantifying})
of the persistence diagrams corresponding to 
each one of the 108 trained WResNets. In Fig.~\ref{fig:total_pers} we plot these values as functions of the test loss at optimum and color the points according to the value of weight decay used during training to reach those points. The first thing we observe is that optima surrounded by regions of high topological activity tend to have a higher loss value at the optima, while low-loss optima have a lower associated total persistence. This further confirms the idea that good generalization optima are surrounded by relatively flat loss-landscape regions while bad generalization optima tend to be situated in regions with many non-convexities. Furthermore we observe that optima found with the most aggressive weight decay (namely 0.001) are surrounded by regions of relatively low topological activity.  Optima reached without the use of weight decay on the other hand are associated with the highest levels of total persistence. These results seem to suggest that the use of weight decay, an efficient regularization method, allows optimizers to find minima on low-loss manifolds with low-persistence topological features. Past results have linked the use of regularization techniques to finding good generalization minima surrounded by flat regions, i.e. regions of low geometrical activity. Here we have expanded on these results by showing that the topological activity in those regions is also relatively low when compared to regions surrounding optima found without regularization.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commented text from the NeurIPS submission
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/different_phate_embeds_loss_level.png}
%     \caption{(PLACEHOLDER FIGURE, NOT ALL PLOTS LOOK LIKE THIS + NEED TO WAIT FOR NEW JUMP AND RETRAIN DATA) 2D PHATE embeddings (top row) of the points in parameter space of two Wide-ResNets sampled with the jump and retrain procedure, and the persistence diagrams (bottom row) of a loss-level filtration computed from the connectivity matrix of a 10-NN graph using the PHATE diffusion potentials as distances. The two neural networks (left and right) have different depths and widths and were trained through different procedures and thus reached different performance levels, 84\% test accuracy for the network on the left and 94\% for the one on the right. Both PHATE and the topological features of the loss landscape seem to differentiate these two networks which have very different generalization capabilities. This suggests that the geometric and topological features of the loss landscape region surrounding an optimum depend on model architecture, training procedure and the network's ability to generalize learning to unseen data.}
%     \label{fig:tda_characterization}
% \end{figure}


%Visualizing the data from the other sampling procedures is not as informative since data sampled around different minima have the same low dimensional embeddings due to the rigid structure of these procedures.
% Running PHATE on the points sampled with the jump and retrain procedures allowed us to visualize and compare the regions in parameter space surrounding the minima of the various networks trained, which all achieved ~0 loss on their respective training sets. Our visualization method reveal stark differences  between  neural  network  configurations  that  memorize  (or  overfit)  versus  ones  that generalize. Visualizing the data from the other sampling procedures is not as informative since regions surrounding different minima have the same low dimensional embeddings due to the rigid nature of the loss
%
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/generalization_memorization_figure.png}
%     \caption{2D PHATE embeddings of the jump and retrain experiment conducted on one good (\textbf{a,d}) and one bad (\textbf{b,e}) generalization minima that achieve 94.39\% and 87.29\% accuracy on the test data respectively, as well as one memorization minimum (\textbf{c,f}). The initial points of the jumps (before retraining) are marked by diamonds of different colors based on $step\_size$ in all plots. All trajectories are colored by their respective direction of the initial jump. Plots \textbf{a,b,c} have ascending hue, meaning the color gets darker as retraining progresses. Plots \textbf{d,e,f} have descending hue, meaning the color gets whiter as retraining progresses. In \textbf{d} and \textbf{e} the points are colored by the direction ($seed$) of the jumps in parameter space and the color grows darker as retraining progresses. In contrast to more continuous trajectories returning to near the optimum in the good generalization case, memorization displays a more random pattern where weights move out before moving back, often switching direction during retraining. Bad generalization appears to be more similar to memorization, where no continuous trajectories were observed. See Appendix \ref{a:generalization_hi_res} for a higher resolution version.}
    
%     \label{fig:generalization}
% \end{figure}

%the flat region surrounding the minimum is wide enough that they return to it. Moreover, they tend to return in the same direction they were pushed out, leading to a star shaped convergence pattern. Such a structure is the high-dimensional equivalent to a ``wide valley'' described in past work studying flatness of optima. While the starting points are all set on five distinct directions from the minimum, the plotted retraining trajectories are not restricted to any subspace of the parameter space.

% Robustness
% One of the main problems encountered in previous attempts to visualize ANN loss landscapes resides in the difficulty of comparing them across tasks and initializations. We verified that our visualization method, applied to points sampled with the jump and retrain procedure, alleviates this concern by training multiple WResNet28-2 networks starting from different parameter initializations. Further, we also trained a similar network on the CIFAR100 dataset, following a similar training procedure. Since CIFAR100 poses a significantly harder classification task than CIFAR10, our networks only reaches \textasciitilde60\% test accuracy for the bad optimum, and \textasciitilde70\% test accuracy for the good optimum. This is just a reflection of the complexity of the task, with better accuracy requiring a better fine-tuning of the architecture and the training procedure. The plots for different initializations of the WResNet28-2 are consistently showing the same star-shaped patterns, characterizing the retraining trajectories surrounding minima that generalize well. The plots for the bad minima also share a similar pattern, not only across initialization but also across tasks. These results are shown Appendix \ref{a:robustness_hi_res}.

% Strikingly, the star-shaped pattern is even better defined in Fig.~\ref{fig:robustness}f, corresponding to the good optimum of WResNet28-2 trained on CIFAR100. This offers a key insight into the effect of regularization on the geometric characteristics of the found minima. It seems that regularization techniques enhance generalization by forcing the optimizer into wider valleys.

%The total persistence acts as a summary of the topological features, with a bigger value signifying the presence of topological features with greater persistence.
%Furthermore we observe that the use of regularization techniques, in this case weight decay, allows the optimizers to find optima in regions with less topological activity. The optima found with the most aggressive weight decay (0.001) are surrounded by regions of relatively low topological activity while optima reached without weight decay are associated with the highest levels of total persistence.

==> neurips2021_files/sections_neurips_clean/6_discussion_conclusion.tex <==
\vspace{-5pt}
\section{Discussion and conclusion}
\vspace{-7pt}
We propose a novel approach to dynamically sample the loss landscapes of deep learning models which takes theoretical inspiration from the fields of Riemannian geometry and dynamical systems. Our sampling method efficiently samples points form the low-loss manifolds surrounding minima found through gradient descent. The resulting sampled data holds more information than past loss landscape sampling methods about the geometry of the loss landscape, the network ability to generalize at the optimum and the training procedure and regularization used to reach that optimum. We then present a new loss landscape visualization method based on the state-of-the-art PHATE dimensionality reduction method, which is able to reconstruct the high-dimensional trajectories sampled in two dimensional representations. Our approach enables geometric exploration of the sampled manifolds and regions surrounding generalization and memorization optima, found via ANN training, to provide insight into generalization capabilities and training of the network. Finally, topological data analysis enables us to characterize these regions through the computation of their topological features. We found that weight decay, a powerful regularization technique, allows ANN optimizers to find minima in regions of lower topological activity. An interesting research direction would be to try to apply dimensionality reduction techniques that better take into account the time dependency of the data. We expect in future work our sampling, visualization and topological characterization approaches to enable more methodical paradigms for the development of deep models that generalize better, train faster, and to provide fundamental understanding of their capabilities.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commented text from the NeurIPS submission
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%We proposed a novel approach to visualize ANN loss landscapes based on the state-of-the-art PHATE dimensionality reduction, which is able to capture branch-like structures in high-dimensional data in two dimensional representations. Our approach enables geometric exploration of retrained trajectories surrounding generalization and memorization optima, found via ANN training, to provide insight into generalization capabilities of the network. Further, it enables meaningful comparison of training trajectories across optimizers. Finally, our proposed paradigm is demonstrably consistent and robust across initializations and supervised learning tasks. We expect in future work this visualization approach to enable more methodical paradigms for the development of deep models that generalize better, train faster, and provide fundamental understanding of their capabilities.

% The optimization landscape of loss functions lies at the heart of (almost) every modern deep learning task. Despite its ubiquity, we have little understanding of how this complex high-dimensional structure affects our models, their training and their performance. What little understanding we do have, however, shows highly relevant links between loss-landscape geometry and network abilities to train and generalize well. We believe the study of loss-landscape characteristics is a promising research direction that has the potential for promoting better fundamental understanding of deep learning. Furthermore, advances in this direction will most likely make use of increasingly complex data exploration tools that extract relevant geometric and topological characteristics of ANN training dynamics. Our proposed visualization method is a step in this direction, which sets the stage for more methodical paradigms to support the development of deep models that generalize better, train faster, and provide fundamental understanding of their capabilities.

==> neurips2021_files/sections_neurips_clean/acknowledgements.tex <==
\section{Acknowledgmentas}
This work was partially funded by: Canada CIFAR AI Chair [G.W., G.L.], NSERC Discovery Grant RGPIN-2018-04821 [G.L.], Samsung Research Support [G.L.], NSERC CGS M scholarship [S.H.]. 
%
The content is solely the responsibility of the authors and does not necessarily represent the official views of the funding agencies.

==> neurips2021_files/sections_neurips_clean/related_work.tex <==
\vspace{-5pt}
\section{Related work}\label{s:related_work}
\vspace{-7pt}
\subsection{Loss landscape visualization}\label{ss:ll_visualization}
%
Loss landscape visualization methods have been proposed in numerous contexts. \citet{goodfellow2014qualitatively} proposed the ``linear path experiment'' where the loss of an ANN is evaluated at a series of points $\theta=(1-\alpha)\theta_i + \alpha \theta_f$ for different values of $\alpha \in [0,1]$ and $\theta_i,\theta_f$ corresponding to the initial parameters of the model and the found optima in parameter space respectively. This one-dimensional linear interpolation method has allowed them to show that popular state of the art ANNs typically do not encounter significant obstacles along a straight path from initialization to convergent solution. They also used the method to visualize the loss along directions connecting two distinct minima and to show that these are linearly separated by a region of higher valued loss.

This method was further developed by \citet{im2016empirical_loss_surfaces}, who adapted it to enable the visualization of two-dimensional projections of the loss-landscape using barycentric and bilinear interpolation for groups of three or four points in parameter space. This analysis method has allowed them to establish that despite starting with the same parameter initialization, different optimization algorithms find different minima. Furthermore, they noticed that the loss-landscape around minima have characteristic shapes that are optimizer-specific and that batch-normalization smoothens the loss function.

More recently, \citet{Goldstein_LL_NIPS2018_7875} have addressed the \textit{scale invariance} and \textit{network symmetries} problems discussed in \citet{neyshabur2017exploring} and \citet{dinh2017sharp_minima_gen}, which prevented meaningful comparisons between loss-landscape plots from different networks. They proposed 1D and 2D linear interpolation plots, similar to past techniques, but where they used filter-wise normalized directions to remove the scaling effect. This method has allowed them to visualize and compare the regions on the loss-landscape surrounding minima coming from multiple networks in a meaningful way and to correlate the ``flatness'' of the region to the generalization capabilities of the corresponding network. Furthermore, they studied the effects of the network depth, width and the presence of skip connections on the geometry of the loss-landscape and on network generalization. %They also proposed using normalized PCA directions to plot training trajectories in two dimensions.

\subsection{Generalization and importance of studying the loss landscape}
Ensuring that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. The idea that a network's ability to generalize is linked to the geometry of the loss landscape around the optima was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers~\citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Following the underlying idea of these propositions, we believe that studying the geometry of the loss landscape around minima has the potential of uncovering key characteristics about the network's ability to generalize. 

Furthermore, the importance of loss landscape visualization methods like the one presented in this paper increases with the growing scientific community interest in furthering our understanding of ANNs. As our understanding of this landscape gets deeper, we start uncovering more and more high-dimensional and complex geometric and topological characteristics. For instance, \citet{essentially_no_barriers} have found nonlinear pathways in parameter space connecting distinct minima, along which the training and test errors remain small and losses are consistently low. This suggests that minima are not situated in isolated valleys but rather on connected manifolds representing low loss regions. However, such characteristics are intrinsically high-dimensional, making linear methods inadequate to visualize these structures. Even in standard applications of the linear methods one inevitably asks if the thousands (or even millions) of unseen directions do not hide critical features of the landscape, and if the visualized linear path is relevant to what happened during training.

\subsection{Manifold learning and topological data analysis}
In this paper, we suggest the use of modern manifold learning and topological data analysis techniques to study the complex loss landscape of ANNs. Manifold learning techniques have been extensively used in recent years to successfully study the internal learned representations of deep networks and highlight their complex geometric structures and intrinsic dimensionality \citep{gigante2019visualizing, horoi2020internal, recanatesi2018signatures, farrell2019dynamic, maheswaranathan2019universality}. Here we further advance theses lines of work to provide new applications and insights in the study of ANN optimization and generalization.

To our knowledge, this is the first time topological data analysis (TDA) has been applied to the study of ANN loss landscapes. 
However, the application of algebraic topology to the analysis of real-valued functions defined on manifolds is not novel, and is in fact at the heart of Morse theory, developed by Marston Morse and others during the 20$^{\text{th}}$ century~\citep{morse1925relations, milnor2016morse}. 
More recently, numerous efficient computational algorithms for solving concrete problems related to algebraic topology have been developed in the field of computational topology \citep{Edelsbrunner10}.
A particular problem that can be solved through the use of TDA algorithms is the topological characterization of critical points of real-valued functions defined on manifolds \citep{Gyulassy08, Gyulassy2006topological, bremer2004topological}. If the ambient dimension of the manifold is low~(2D or 3D), such a characterization gives rise to a decomposition of a function in terms of regions of similar gradient behavior~(the classical example is a function with two peaks defined on $\mathbf{R}^2$; here, there would be a decomposition into regions that measure which peak is ``closer''). This decomposition is known as the Morse--Smale complex. 
The Morse--Smale complex can be computed from the critical points of the respective function and its unstable manifolds as defined by the dynamics of gradient descent~(or ascent). 
The hierarchical structure of the complexes and the function's topological features are found by considering the succession of critical points and unstable manifolds in the increasing sequence of the function's sublevel sets, i.e., the set of all points on the manifold whose function value is less than or equal to a pre-defined threshold. 
%
The difference between the function values of different critical points---equivalently, this is the difference between the ``appearance'' and ``disappearance'' of a topological feautre---is referred to as the \emph{persistence}. Persistence  can be used to simplify a given function by smoothing out features; this is typically achieved by cancelling related pairs of critical points whose persistence fails to satisfy a certain simplification threshold.
Such analysis methods have been successfully applied in the field of electrochemistry, for instance, to characterize the topology of energy landscapes of different molecules \citep{Gyulassy2006topological, bremer2004topological}. 
This directly relates to our work since the loss-landscape associates a loss value to each point in the parameter space of the ANN and we wish to characterize the topology of this landscape. The primary difference to existing work is that we are dealing with a manifold whose~(ambient) dimension is much higher, thus precluding the analytical calculation of the Morse--Smale complex.

%
% \subsection{Generalization and sharpness of the landscape at the optimum}
% Making sure that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. It is so important that oftentimes large fractions of the scarcely available data are not used for training but rather for testing, to ensure that models indeed learn to solve the task in a relevant manner without overfitting their training data. Arguably one of the most important and general questions in machine learning at the moment is: by looking only at a given trained model and its training data, can we predict how well the model will perform on unseen data? There was even an entire NeurIPS 2020 competition entirely focused on answering this question \citep{pgdl_neurips2020}. 
%
% Previous work offers a partial and vague answer to this question by linking the ``flatness'' of neural network optima to the extent to which the network is able to generalize. This idea was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers \citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Following the underlying idea of these propositions, we believe that studying the geometry of the loss landscape around minima has the potential of uncovering key characteristics about the network's ability to generalize.

% \subsection{Importance of studying the loss landscape}
% In this paper, we suggest the use of modern manifold learning and topological data analysis techniques to study the complex loss-landscape of ANNs. Manifold learning techniques have been extensively used in recent years to successfully study the internal learned representations of deep networks and highlight their complex geometric structures and intrinsic dimensionality \citep{gigante2019visualizing, horoi2020internal, recanatesi2018signatures, farrell2019dynamic, maheswaranathan2019universality}. TDA on the other hand has recently been applied to analyze brain imaging data \citet{rieck2020_fmri_cubical} and has been gaining popularity in the field of deep learning \citet{}. Here we further advance theses lines of work to provide new applications and insights in the study of ANN optimization and generalization.

==> neurips2021_files/sections_neurips_clean/related_work_short.tex <==
\vspace{-7pt}
\section{Related work}\label{s:related_work}
\vspace{-10pt}
% \subsection{Loss landscape visualization}\label{ss:ll_visualization}
%
Loss landscape visualization methods have been proposed in numerous contexts. \citet{goodfellow2014qualitatively} proposed the ``linear path experiment'' where the loss of an ANN is evaluated at a series of points $\theta=(1-\alpha)\theta_i + \alpha \theta_f$ for different values of $\alpha \in [0,1]$ and $\theta_i,\theta_f$ corresponding to the initialization and optimum respectively. This one-dimensional linear interpolation method has allowed them to show that popular state of the art ANNs typically do not encounter obstacles along a straight path from initialization to convergent solution and that distinct minima are linearly separated by a region of higher valued loss. This method was further developed by \cite{im2016empirical_loss_surfaces}, who adapted it to enable the visualization of two-dimensional projections of the loss-landscape. This analysis method has allowed them to establish that despite starting with the same parameter initialization, different optimization algorithms find different minima surrounded by regions of characteristic shapes that are optimizer-specific. More recently, \citet{Goldstein_LL_NIPS2018_7875} have addressed the \textit{scale invariance} \citep{neyshabur2017exploring} and \textit{network symmetries} \citep{dinh2017sharp_minima_gen} problems  which prevented meaningful comparisons between loss-landscape plots from different networks. They proposed 1D and 2D linear interpolation plots where they used filter-wise normalized directions to remove the scaling effect. This allowed them to visualize and compare the regions on the loss-landscape surrounding minima coming from multiple networks.
%in a meaningful way. 
% and to correlate the ``flatness'' of the region to the generalization capabilities of the corresponding network.% Furthermore, they studied the effects of the network depth, width and the presence of skip connections on the geometry of the loss-landscape and on network generalization. %They also proposed using normalized PCA directions to plot training trajectories in two dimensions.

% Ensuring that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. The idea that a network's ability to generalize is linked to the geometry of the loss landscape around the optima was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers \citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Following the underlying idea of these propositions, we believe that studying the geometry of the loss landscape around minima has the potential of uncovering key characteristics about the network's ability to generalize. 

% Furthermore, the importance of loss landscape visualization methods like the one presented in this paper increases with the growing scientific community interest in furthering our understanding of ANNs. As our understanding of this landscape gets deeper, we start uncovering more and more high-dimensional and complex geometric and topological characteristics. For instance, \citet{essentially_no_barriers} have found nonlinear pathways in parameter space connecting distinct minima, along which the training and test errors remain small and losses are consistently low. This suggests that minima are not situated in isolated valleys but rather on connected manifolds representing low loss regions. However, such characteristics are intrinsically high-dimensional, making linear methods inadequate to visualize these structures. Even in standard applications of the linear methods one inevitably asks if the thousands (or even millions) of unseen directions do not hide critical features of the landscape, and if the visualized linear path is relevant to what happened during training.

% In this paper, we suggest the use of modern manifold learning and topological data analysis techniques to study the complex loss landscape of ANNs. Manifold learning techniques have been extensively used in recent years to successfully study the internal learned representations of deep networks and highlight their complex geometric structures and intrinsic dimensionality \citep{gigante2019visualizing, horoi2020internal, recanatesi2018signatures, farrell2019dynamic, maheswaranathan2019universality}. Here we further advance theses lines of work to provide new applications and insights in the study of ANN optimization and generalization.

%
% \subsection{Generalization and sharpness of the landscape at the optimum}
% Making sure that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. It is so important that oftentimes large fractions of the scarcely available data are not used for training but rather for testing, to ensure that models indeed learn to solve the task in a relevant manner without overfitting their training data. Arguably one of the most important and general questions in machine learning at the moment is: by looking only at a given trained model and its training data, can we predict how well the model will perform on unseen data? There was even an entire NeurIPS 2020 competition entirely focused on answering this question \citep{pgdl_neurips2020}. 
%
% Previous work offers a partial and vague answer to this question by linking the ``flatness'' of neural network optima to the extent to which the network is able to generalize. This idea was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers \citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Following the underlying idea of these propositions, we believe that studying the geometry of the loss landscape around minima has the potential of uncovering key characteristics about the network's ability to generalize.

% \subsection{Importance of studying the loss landscape}

% In this paper, we suggest the use of modern manifold learning and topological data analysis techniques to study the complex loss-landscape of ANNs. Manifold learning techniques have been extensively used in recent years to successfully study the internal learned representations of deep networks and highlight their complex geometric structures and intrinsic dimensionality \citep{gigante2019visualizing, horoi2020internal, recanatesi2018signatures, farrell2019dynamic, maheswaranathan2019universality}. TDA on the other hand has recently been applied to analyze brain imaging data \citet{rieck2020_fmri_cubical} and has been gaining popularity in the field of deep learning \citet{}. Here we further advance theses lines of work to provide new applications and insights in the study of ANN optimization and generalization.

==> obsolete files/generalization.tex <==
\subsection{Generalization vs. Memorization}\label{ss:generalization}
Making sure that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. It is so important that oftentimes large fractions of the scarcely available data are not used for training but rather for testing, to ensure that models indeed learn to solve the task in a relevant manner without overfitting their training data. Arguably one of the most important and general questions in machine learning at the moment is: by looking only at a given trained model and its training data, can we predict how well the model will perform on unseen data? There was even an entire NeurIPS 2020 competition entirely focused on answering this question \citep{pgdl_neurips2020}. 

Previous work offers a partial and vague answer to this question by linking the ``flatness'' of neural network optima to the extent to which the network is able to generalize. This idea was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers \citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Here, we show that jump-and-retrain experiments combined with our visualization method reveal stark differences between neural network configurations that memorize (or overfit) versus ones that generalize. 

For our empirical results we trained multiple WResNet28-2 networks (wide ResNet of depth 28 and 2 times as wide as a standard ResNet \citep{resnet}) presented in \cite{wide_resnet} on the CIFAR10 dataset \citep{cifar10} using batches of size 128 for 200 epochs with the SGD optimizer with 0.9 momentum and a learning rate of 0.1 which decays by a factor of 10 at epoch 150. In some cases we did not use data augmentation and weight decay and in others we used 1e-4 weight decay and random crops and horizontal flips for the training data. Adding the data augmentation and the weight decay has allowed us to find optima that generalize better, increasing the accuracy on the test data from around 85\% to around 95\%. We will be referring the optima with \textasciitilde95\% test accuracy as ``good optima'' since they generalize better, and that with lower test accuracy as ``bad optima''. Using the same training procedure as the one for the bad optima, we also trained a WResNet28-2 network for memorization by completely randomizing the labels of the training data. This modification was used in \cite{Zhang2017UnderstandingDL,closer_look_memorization, dnns_don't_learn_via_mem} to show that neural networks have the ability to completely memorize the training data sets. We then ran the jump-and-retrain experiment for these three types of minima and visualized the results using PHATE in Figure \ref{fig:generalization}. This allows us to analyze and compare the regions in parameter space around the good, bad and memorization minima, which all achieve \textasciitilde0 loss on their respective training sets.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/generalization_memorization_figure.png}
    \caption{2D PHATE embeddings of the jump and retrain experiment conducted on one good (\textbf{a,d}) and one bad (\textbf{b,e}) generalization minima that achieve 94.39\% and 87.29\% accuracy on the test data respectively, as well as one memorization minimum (\textbf{c,f}). The initial points of the jumps (before retraining) are marked by diamonds of different colors based on $step\_size$ in all plots. All trajectories are colored by their respective direction of the initial jump. Plots \textbf{a,b,c} have ascending hue, meaning the color gets darker as retraining progresses. Plots \textbf{d,e,f} have descending hue, meaning the color gets whiter as retraining progresses. In \textbf{d} and \textbf{e} the points are colored by the direction ($seed$) of the jumps in parameter space and the color grows darker as retraining progresses. In contrast to more continuous trajectories returning to near the optimum in the good generalization case, memorization displays a more random pattern where weights move out before moving back, often switching direction during retraining. Bad generalization appears to be more similar to memorization, where no continuous trajectories were observed. See Appendix \ref{a:generalization_hi_res} for a higher resolution version.}
    
    \label{fig:generalization}
\end{figure}

Despite having only a \textasciitilde7\% difference in their accuracy on the test data set, the PHATE embedding of the trajectories surrounding each generalization minimum is significantly different as seen in Fig.~\ref{fig:generalization}d. The minimum that shows good generalization has a distinctive star or flower shaped pattern. This pattern in a jump-and-retrain experiment indicates that even when points are thrown far from the minimum, the landscape is wide enough that they return to it. Moreover, they tend to return in the same direction they were pushed out, leading to a flower-petal convergence pattern. Such a structure is the high-dimensional equivalent to a ``wide valley'' described in past work studying flatness of optima. While the starting points are all set on five distinct directions from the minimum, the plotted retraining trajectories are not restricted to any subspace of the parameter space.

In the bad minimum on the other hand, the trajectories start off near the middle of the plot (darker points in the middle of Fig.~\ref{fig:generalization}b) but during the retraining, the trajectories diverge toward the edges before coming back towards the middle of the plot. This outward movement is stark contrast with the consistent retraining trajectories surrounding the good generalization minimum, which immediately return to the valley. This indicates that the region around the bad-generalization minimum is most probably not a wide (or flat) high-dimensional valley and contains a nonnegligible amount of nonconvexities, preventing training trajectories to systematically converge towards the minimum.  The ``memorization'' minimum plot Fig.~\ref{fig:generalization}c looks similar to the bad generalization plot, with trajectories that go outward at small step sizes of the "jump." However, curiously at larger step sizes of the "jump," the trajectories seem to return without going outward first,  but they do not return immediately, i.e., they show some lateral movement, potentially indicating bumpiness in the landscape that they are avoiding.  Thus we see a clear pattern in  the good generalization minima of inward movement upon the jump and retrain, and more outward behavior in the bad generalization and memorizations. See supplemental video for an animation of these trajectories, and Appendix \ref{a:generalization_hi_res} for trajectories colored by loss.



==> obsolete files/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> obsolete files/optimization.tex <==
\subsection{Optimization}\label{ss:optimization}

We analyzed three stochastic gradient-descent optimization methods commonly used for training ANNs: SGD (vanilla), SGD with momentum (SGD{\textunderscore}M), and Adam. The major difference is that Adam uses adaptive step sizes based off previous iterations while SGD and SGD{\textunderscore}M use fixed step sizes. We are interested in answering questions including how the network evolves during training with different optimizer and whether different optima are reached at the end of training.

% Stochastic gradient descent (SGD) with momentum has been shown to train neural networks to better performance than Hessian-Free optimizations. We are interested in answering questions including whether the superior performance is achieved by reaching a different, maybe better, optimum when more advanced optimizer are utilized and how the network evolves during training with different optimizer. We visualize the parameters at the end of training.

%\subsubsection{Experiments}
We trained Wide-ResNet networks of depth 28 and twice as wide, which is the same as in the previous section. 
%Three optimizers are compared including 1) baseline optimizer of SGD without momemtum (SGD), 2) SGD with momentum 0.9 (SGD\_M) and 3) Adam. 
%CGOpt similar to Adam but worse performance ($87\%$)
The same initial learning rate of 0.1 and learning rate decay schedule is employed with each optimizer, data augmentation is used to assist training while no weight decay was used. All experiments achieve close to $100\%$ training accuracy and $> 90\% $ test accuracy. A fixed set of five seeds is used across optimizers. 

% \subsubsection{Results}
First we examine individual trajectories of network weights from the same seed using different optimizers (Fig.~\ref{fig:optim_compare_single}). Compared to the smooth trajectory from using Adam, SGD with or without momentum seems to exhibit scattered patterns. It should be noted that the magnitudes of network weights learned by Adam are much larger than by SGD or SGD{\textunderscore}M (Appendix~\ref{a:optim_weights_norm}). The evolution and resulting network weights from the Adam optimizer appears to differ more significantly from SGD or SGD\_M, where the resulting parameters appear to be further away from the initialization. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/fig_optimizers_single_run (4).png}
    \caption{Comparing PHATE embedding of network weights during training using different optimizers. The same seed was used across optimizers, Adam produces a more smooth trajectory. }
    \label{fig:optim_compare_single}
    \vspace{-0.15 in}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/fig_optimizer_compare (1).png}
%     \caption{PHATE embedding of network parameters during training using different optimizers. }
%     \label{fig:optim_compare}
% \end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/fig_optimizer_compare_cos (5).png}
    \caption{PHATE embedding (cosine distance) of network parameters during training using different optimizers (SGD, SGD\_M, and Adam). The five initialization are marked by golden stars. (a),(b)Different optimization algorithms reach distinct minima that all lie in a disc-shaped region. ADAM seems to search an orthogonal space of the loss landscape from SGD with momentum, as seen by the "disappearance" of the trajectory, (c) The Adam trajectories, plotted by themselves are continuous, however distances between final weights reached by Adam are much larger than other optimizers.See Appendix~\ref{a:optim_comparison_hi_res} for higher resolution images}
    \label{fig:optim_compare_cos}
    \vspace{-0.1 in}
\end{figure}

In Fig.~\ref{fig:optim_compare_cos} the distinctiveness between optima reached from different initializations and optimizers are clearly shown. We see in the Fig.~\ref{fig:optim_compare_cos}(a) that when starting from the same seed, SGD and SGD with momentum travel in similar directions. However, we see a shorter and straighter training path with momentum. Without momentum, a similar minima is reached. However, the path towards the minima is longer with more moves sideways, indicating that the space is searched less effectively.  In  Fig.~\ref{fig:optim_compare_cos}(b) the fact that Adam travels so far in the weight space, causes the initial points look very close together. From the initial points, the SGD with momentum travels in shorter paths towards different minima. However, Adam seems to exhibit a disconnected jump, potentially flying off into an orthogonal space to what is visualized, but interestingly returning to the same region of minima as SGD\_M. The seemingly discontinuity of the trajectories in the middle plots indicates that Adam searches space very differently than SGD. Fig.~\ref{fig:optim_compare_cos}(c) shows that the Adam trajectories are indeed connected in a continuous line, so the trajectory itself is not discontinuous, but rather in a different subspace than the SGD\_M trajectory. 

% \textcolor{red}{TODO:it could be adjusted by adding weight decay Adam weight decay or L2 reglarization is different from basic SGD, needs more looking into}. 
%The scaling of weights may be playing a role here. It is arguable that smaller weights may be more sensitive to perturbations even if they achieve better training/testing accuracy, and visualizing network weights using PHATE can guide selection of optimizer. 

%All experiments achieve similar test accuracy of $>90\%$. However, the minima constructed from five random initializations and through different optimization algorithms appear to be distinct. We verified that for each set of networks trained using the same optimizer and different initialization, the overlap of samples that are misclassified at two minima is around $50\%$ to $60\%$. It should be noted that the distance on the inferred manifold does not imply the level of distinctiveness in terms of overlapping misclassification.

%When cosine distance is used in PHATE as in Figure~\ref{fig:optim_compare_cos}, we can see that comparing to SGD and SGD\_M, Adam leads to bigger jumps in the learning trajectories. Moreover, the distances between final weights by Adam are much larger than that between the initial weights from different random initialization (Fig.~\ref{fig:optim_compare_cos}(c)). Indeed, different optima are reached with different optimizers. Despite the large variation in actual weights, PHATE with cosine distance allows visualizing that all trajectories end in a disc-shaped area in 2-dimension.

==> obsolete files/results_old_version.tex <==
\section{Results}\label{s:results}
% \subsection{Visualizing the loss landscape surrounding minima}
% \subsection{Linking the topological features of the loss landscape to training hyperparameters and generalization}

\subsection{Experimental setup}\label{ss:experimental setup}
Since the objects of interest of this project are trained ANNs and their optimum found through training, we have trained multiple wide ResNets \citep{wide_resnet} on the CIFAR10 image classification task \citep{cifar10} from initialization to optimum. The networks trained had depth $\in \{10, 16, 22\}$, width $\in\{1,2\}$ and were trained with a combination of the following training hyperparameters: batch size $\in\{32, 128, 512\}$, weight decay $\in\{0, 0.0001, 0.001\}$ and either with or without data augmentation (random horizontal flips and crops). One network was trained for every possible combination of these values for a total of 108 WResNets, all having the same initialization. All networks were trained for 200 epochs using SGD with 0.9 momentum and a learning rate of 0.1 which was multiplied by 0.1 at epochs 100, 150 and 185.
%The test accuracy of the networks greatly varied according to the values of these design choices and training hyperparameters.

We also trained a limited amount of WResNet28-2 networks on CIFAR10 using batches of size 128 for 200 epochs with the same optimizer. In some cases we did not use data augmentation and weight decay and in others we used 1e-4 weight decay and random crops and horizontal flips for the training data. Adding the data augmentation and the weight decay has allowed us to find optima that generalize better, increasing the accuracy on the test data from around 85\% to around 95\%. We will be referring the optima with \textasciitilde95\% test accuracy as ``good optima'' since they generalize better, and that with lower test accuracy as ``bad optima''. Using the same training procedure as the one for the bad optima, we also trained a WResNet28-2 network for memorization by completely randomizing the labels of the training data. This modification was used in \cite{Zhang2017UnderstandingDL,closer_look_memorization, dnns_don't_learn_via_mem} to show that neural networks have the ability to completely memorize the training data sets. These WResNet28-2 networks were specifically trained to compare between the good, the bad and the memorization optima.

% Once this ensemble of trained networks and their respective optimums was obtained it was possible to sample the loss landscape region surrounding the optimums using each one of the presented procedures. For the jump and retrain sampling, after each ''jump'' every network was retrained for 40 epochs using a batch-size of 128 and the SGD optimizer with 0.9 momentum and a learning rate of 0.01, no weight decay or data augmentation was used during the retraining. This retraining procedure was fixed for all networks, independently of the original training procedure used to find the optimums.

% \paragraph{Libraries and code}
% All the experiments were ran with Pytorch. The code for training the WResNet models was adapted from \cite{github} relating to the paper \cite{} made available through the MIT license. The code for filter-normalizing random directions and updating a model's parameters was adapted from \cite{github} relating to the paper \cite{} made available through the MIT license. 

\subsection{Effectiveness of the jump and retrain sampling procedure}\label{ss:results_sampling}
In order to see if the sampled data holds information about the networks ability to generalize to unseen data we analyzed it in a predictive setting and formulated the following classification task. We used the sampled loss and accuracy values as features and we separated the trained WResNet models into 5 (almost) equally-sized ``generalization'' classes according to the value of the loss on the test set at optimum. The \textasciitilde20\% of networks with the lowest test loss at optimum were in class 1, and so on. We then trained 11 simple classifiers to predict the generalization class of each network from the training loss and accuracy features. The classifiers were trained and evaluated using 10-fold cross validation. It is important to note that the 11 classifiers were not tuned to any of the features to not favor any of the sampling procedures.
%
%The 11 classifiers were: k-NN classifier with k=5, linear SVM, RBF kernel SVM, Gaussian Process classifier, decision tree, random forest with 100 trees, MLP classifier with 1 hidden layer of 100 ReLU neurons trained with ADAM, AdaBoost classifier with base classifier a decision tree with depth 1, Gaussian Naive Bayes, Multinomial Naive Bayes and a Quadratic Discriminant Analysis classifier. The classifiers were trained and evaluated using 10-fold cross validation.
%

In order to evaluate the effectiveness of the jump and retrain sampling procedure we compared the results to those obtained with two other sampling procedures. The first sampling procedure considered, that we name grid sampling is directly inspired by the 1D or 2D linear interpolations used in past visualization methods. We randomly choose 3 vectors starting from $\theta_o$ and construct a 3D grid using the 3 vectors as basis. The loss and accuracy on the training set is then evaluated at all points on the grid. The second comparison sampling procedure, that we call naive sampling, evaluates the loss in random directions ($\theta_i$) and multiple step sizes ($c$) in these directions from the optimum, i.e. it evaluates the loss at $\theta_o + c\theta_i$. This was inspired by the idea that using more directions and step sizes when sampling, without the grid-like structure, could be more informative since it explores a greater number of directions in parameter space.
%is inspirede hypothesize that there are more efficient ways to sample the loss landscape in a way that is evocative of the network's ability to generalize. We propose the idea that using more directions and step sizes when sampling, without the grid-like structure, could be more informative since it explores a greater number of directions in parameter space. The naive sampling procedure selects 32 random vectors in parameter space, $\theta_i, i\in\{1,\ldots,32\}$, and evaluates the loss and accuracy on the training set at points corresponding to the sum of the parameters at the optimum and one of these directions multiplied by a step size. In other words we evaluate the loss and accuracy at the points $\theta_o + c\theta_i$ for $c\in\{0.05, 0.1, 0.15, \ldots, 0.95, 1.0\}$ (20 possible values) and $i\in\{1,\ldots, 32\}$.
%
All three considered methods sample 640 points from the loss landscape excluding the optimum itself. While the number of points sampled is somewhat arbitrary, it is important to compare the methods with the same number of points. We found 640 points to hold enough information about the loss landscape while still being small enough for our experiments to run without any major computational challenges. Because of the effectiveness of the filter-wise normalization presented in \cite{Goldstein_LL_NIPS2018_7875}, we normalize all random vectors in parameter space in this manner. As a control experiment we also trained the same classifiers on scrambled versions of the features to make sure that the classifiers are not overfitting the data and to evaluate the impact of the features distributions alone. The mean and standard deviation (TO BE CHANGED TO STANDARD ERROR) across the 11 classifiers are shown in Table \ref{tab:generalization}.


\begin{table}
\centering
\caption{Mean and standard deviation of the 11 classifiers accuracies on the 5 class generalization classification task with different features (TEMPORARY DATA).}
\label{tab:generalization}
 \begin{tabular}{|M{7.4cm}|M{2.6cm}|}
 \hline
 Features & Mean and s.d. (\%) \\
 \hline
 Theoretical random (1/\#classes) & 20.0\\
\hline \hline
 Grid sampling,  train loss and accuracy values & 30.1 $\pm$ 8.9 \\ 
 \hline
 Naive sampling, train loss and accuracy values & 31.8 $\pm$ 13.4  \\
 \hline
 J\&R sampling, retrain loss and accuracy values & 31.9 $\pm$ 8.0  \\
 \hline
 J\&R sampling, valid loss and accuracy values & \textbf{39.1} $\pm$ 14.3  \\
 \hline
 Randomized J\&R valid loss and accuracy values & 18.9 $\pm$ 2.4 \\
 \hline
\end{tabular}
\end{table}

% Across the sampling procedures, the loss and accuracy values collected with naive sampling achieve the greatest maximum accuracy on the 5 class generalization classification task, namely 66.7\%. The jump and retrain valid samples achieve slightly less at 63.0\% max accuracy but with a significantly better mean accuracy at 39.1\% than the other features. We remind the reader that the retrain and validation data sets are subsets of the original training data set, i.e. train set = retrain set $\cup$ valid set. The jump and retrain retrain data and grid sampling train data are the worse at predicting generalization with maximum accuracies of 45.4\% and 48.1\% respectively. In all cases the sampling seems to truly hold information about the network generalization capabilities since it performs significantly better than random and then the randomized J\&R features. These results seem to confirm our earlier hypothesis, that grid like sampling is not the most efficient way to sample the loss landscape if we wish to uncover links with the network's ability to generalize. The fact that we can look into multiple directions seem to benefit the naive sampling data.


%We consider the following three sampling procedures designed to explore the loss-landscape region surrounding a given optimum $\theta_o \in \Theta$ found through typical ANN training. 
% The first procedure is inspired by the literature the two others are designed by us, all of them sample 640 points from the loss landscape excluding the optimum itself. While the number of points sampled is somewhat arbitrary, it is important to compare the methods with the same number of points. We found 640 points to hold enough information about the loss landscape while still being small enough for our experiments to run without any major computational challenges. Because of the effectiveness of the filter-wise normalization presented in \cite{Goldstein_LL_NIPS2018_7875}, we normalize all random vectors in parameter space in this manner.

% \paragraph{Grid sampling} 
% Similar to the 1D or 2D linear interpolation used in past visualization methods, we randomly choose 3 vectors starting from $\theta_o$ and construct a 3D grid using the 3 vectors as basis. The loss and accuracy on the training set is then evaluated at all points on the grid. 
% As discussed in the Related Work section, most loss landscape visualization methods are based on 1D or 2D linear interpolations. The loss landscape is in that case sampled by evaluating the loss at equally spaced points from a line or a plane in parameter space, all other dimensions are ignored. We adapt the grid sampling procedure to three dimensions. Three random directions are chosen in parameter space, $\theta_1, \theta_2, \theta_3$, because of the dimensionality of the space these directions are nearly orthogonal with high probability. The loss and accuracy on the training set is evaluated at points in parameter space corresponding to the sum of the parameters at the optimum and linear combinations of these directions, i.e. $\theta_o + c_1\theta_1 + c_2\theta_2 + c_3\theta_3$ with coefficients $c_1\in\{-1.0, -0.8, -0.6, -0.4, -0.2, 0.2, 0.4, 0.6 ,0.8, 1.0\}$ and $c_2, c_3 \in\{-0.8, -0.6, -0.4, -0.2, 0.2, 0.4, 0.6 ,0.8\}$.
% %
% %Certain geometrically inspired methods to evaluate the sharpness of a found minimum rely on computing the Hessian to determine the principal curvatures of the loss landscape at the minimum. However such methods are so computationally expensive that they are often conducted just at the optimum.

% \paragraph{Naive sampling} The grid structure of the previous sampling procedure makes it easy to construct interpretable plots of the loss landscape for visualization purposes. However, to our knowledge there is no prior result stating that such a rigid sampling of the loss landscape holds the most information about the landscape. We hypothesize that there are more efficient ways to sample the loss landscape in a way that is evocative of the network's ability to generalize. We propose the idea that using more directions and step sizes when sampling, without the grid-like structure, could be more informative since it explores a greater number of directions in parameter space. The naive sampling procedure selects 32 random vectors in parameter space, $\theta_i, i\in\{1,\ldots,32\}$, and evaluates the loss and accuracy on the training set at points corresponding to the sum of the parameters at the optimum and one of these directions multiplied by a step size. In other words we evaluate the loss and accuracy at the points $\theta_o + c\theta_i$ for $c\in\{0.05, 0.1, 0.15, \ldots, 0.95, 1.0\}$ (20 possible values) and $i\in\{1,\ldots, 32\}$.

% \paragraph{Jump and retrain sampling}
% While the two first sampling procedures are very easy to implement and sample the loss in an orderly manner, the information gathered about the loss is not used during the procedure itself. 

\subsection{Visualizing the loss landscape region surrounding optima}\label{ss:results_visualization}
Running PHATE on the points sampled with the jump and retrain procedures allowed us to visualize and compare the regions in parameter space surrounding the minima of the various networks trained, which all achieved \textasciitilde0 loss on their respective training sets. Our visualization method reveal stark differences between neural network configurations that memorize (or overfit) versus ones that generalize.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/generalization_memorization_figure.png}
    \caption{2D PHATE embeddings of the jump and retrain experiment conducted on one good (\textbf{a,d}) and one bad (\textbf{b,e}) generalization minima that achieve 94.39\% and 87.29\% accuracy on the test data respectively, as well as one memorization minimum (\textbf{c,f}). The initial points of the jumps (before retraining) are marked by diamonds of different colors based on $step\_size$ in all plots. All trajectories are colored by their respective direction of the initial jump. Plots \textbf{a,b,c} have ascending hue, meaning the color gets darker as retraining progresses. Plots \textbf{d,e,f} have descending hue, meaning the color gets whiter as retraining progresses. In \textbf{d} and \textbf{e} the points are colored by the direction ($seed$) of the jumps in parameter space and the color grows darker as retraining progresses. In contrast to more continuous trajectories returning to near the optimum in the good generalization case, memorization displays a more random pattern where weights move out before moving back, often switching direction during retraining. Bad generalization appears to be more similar to memorization, where no continuous trajectories were observed. See Appendix \ref{a:generalization_hi_res} for a higher resolution version.}
    
    \label{fig:generalization}
\end{figure}

Despite having only a \textasciitilde7\% difference in their accuracy on the test data set, the PHATE embedding of the trajectories surrounding each generalization minimum is significantly different as seen in Fig.~\ref{fig:generalization}. The minimum that shows good generalization has a distinctive star shaped pattern. This pattern indicates that even when points are thrown far from the minimum, the flat region surrounding the minimum is wide enough that they return to it. Moreover, they tend to return in the same direction they were pushed out, leading to a star shaped convergence pattern. Such a structure is the high-dimensional equivalent to a ``wide valley'' described in past work studying flatness of optima. While the starting points are all set on five distinct directions from the minimum, the plotted retraining trajectories are not restricted to any subspace of the parameter space.

In the bad minimum on the other hand, the trajectories start off near the middle of the plot (darker points in the middle of Fig.~\ref{fig:generalization}b) but during the retraining, the trajectories diverge toward the edges before coming back towards the middle of the plot. This outward movement is stark contrast with the consistent retraining trajectories surrounding the good generalization minimum, which immediately return to the valley. This indicates that the region around the bad-generalization minimum is most probably not a wide (or flat) high-dimensional valley and contains a nonnegligible amount of nonconvexities, preventing training trajectories to systematically converge towards the minimum.  The ``memorization'' minimum plot Fig.~\ref{fig:generalization}c looks similar to the bad generalization plot, with trajectories that go outward at small step sizes of the "jump." However, curiously at larger step sizes of the "jump," the trajectories seem to return without going outward first,  but they do not return immediately, i.e., they show some lateral movement, potentially indicating bumpiness in the landscape that they are avoiding.  Thus we see a clear pattern in  the good generalization minima of inward movement upon the jump and retrain, and more outward behavior in the bad generalization and memorizations. See supplemental video for an animation of these trajectories, and Appendix \ref{a:generalization_hi_res} for trajectories colored by loss.

% Robustness
One of the main problems encountered in previous attempts to visualize ANN loss landscapes resides in the difficulty of comparing them across tasks and initializations. We verified that our visualization method, applied to points sampled with the jump and retrain procedure, alleviates this concern by training multiple WResNet28-2 networks starting from different parameter initializations. Further, we also trained a similar network on the CIFAR100 dataset, following a similar training procedure. Since CIFAR100 poses a significantly harder classification task than CIFAR10, our networks only reaches \textasciitilde60\% test accuracy for the bad optimum, and \textasciitilde70\% test accuracy for the good optimum. This is just a reflection of the complexity of the task, with better accuracy requiring a better fine-tuning of the architecture and the training procedure. The plots for different initializations of the WResNet28-2 are consistently showing the same star-shaped patterns, characterizing the retraining trajectories surrounding minima that generalize well. The plots for the bad minima also share a similar pattern, not only across initialization but also across tasks. These results are shown Appendix \ref{a:robustness_hi_res}.

% Strikingly, the star-shaped pattern is even better defined in Fig.~\ref{fig:robustness}f, corresponding to the good optimum of WResNet28-2 trained on CIFAR100. This offers a key insight into the effect of regularization on the geometric characteristics of the found minima. It seems that regularization techniques enhance generalization by forcing the optimizer into wider valleys.

\subsection{Topological characterization of loss landscape regions}\label{ss:results_tda}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/different_phate_embeds_loss_level.png}
    \caption{(PLACEHOLDER FIGURE, NOT ALL PLOTS LOOK LIKE THIS + NEED TO WAIT FOR NEW JUMP AND RETRAIN DATA) 2D PHATE embeddings (top row) of the points in parameter space of two Wide-ResNets sampled with the jump and retrain procedure, and the persistence diagrams (bottom row) of a loss-level filtration computed from the connectivity matrix of a 10-NN graph using the PHATE diffusion potentials as distances. The two neural networks (left and right) have different depths and widths and were trained through different procedures and thus reached different performance levels, 84\% test accuracy for the network on the left and 94\% for the one on the right. Both PHATE and the topological features of the loss landscape seem to differentiate these two networks which have very different generalization capabilities. This suggests that the geometric and topological features of the loss landscape region surrounding an optimum depend on model architecture, training procedure and the network's ability to generalize learning to unseen data.}
    \label{fig:tda_characterization}
\end{figure}

% \subsection{Generalization}
% In order to see if the sampled data holds information about the networks ability to generalize to unseen data we analyzed it in a predictive setting and formulated the following classification task. We used the sampled loss and accuracy values on the training data set as features and we separated the trained WResNet models into 5 (almost) equally-sized ''generalization'' classes according to the value of the loss on the test set at optimum. The \textasciitilde20\% of networks with the lowest test loss at optimum were in class 1, and so on. We then trained 11 simple classifiers to predict the generalization class of each network
% from the training loss and accuracy features. The 11 classifiers were: k-NN classifier with k=5, linear SVM, RBF kernel SVM, Gaussian Process classifier, decision tree, random forest with 100 trees, MLP classifier with 1 hidden layer of 100 ReLU neurons trained with ADAM, AdaBoost classifier with base classifier a decision tree with depth 1, Gaussian Naive Bayes, Multinomial Naive Bayes and a Quadratic Discriminant Analysis classifier. The classifiers were trained and evaluated using 10-fold cross validation.

% The same analysis set up and classification task were used to evaluate if the topological features extracted held any information about the networks generalization capabilities by using the topological features instead of the loss and accuracy values.  As a control experiment we trained the same classifiers on scrambled versions of the features to make sure that the classifiers are not overfitting the data and to evaluate the impact of the features distributions alone. The maximum, mean and standard deviation across the 11 classifiers are shown in Table \ref{tab:generalization}.

% %In order to verify if the topological features and the loss and accuracy values held complementary information, we used the predictions generated by the best classifiers in both context and trained a decision tree on both the predictions made from the topological features and from the loss and accuracy values.

% \begin{table}
% \centering
% \caption{Maximum, mean and standard deviation of the 11 classifiers accuracies on the 5 class generalization classification task with different features.}
% \label{tab:generalization}
%  \begin{tabular}{|M{7.4cm}|M{2.6 cm}|M{2.6cm}|}
%  \hline
%  Features & Max accuracy (\%) & Mean and s.d. (\%) \\
%  \hline
%  Theoretical random (1/\#classes) & 20.0 & 20.0\\
% \hline \hline
%  Grid sampling,  train loss and accuracy values & 48.1 & 30.1 $\pm$ 8.9 \\ 
%  \hline
%  Naive sampling, train loss and accuracy values & \textbf{66.7} & 31.8 $\pm$ 13.4  \\
%  \hline
%  J\&R sampling, retrain loss and accuracy values & 45.4 & 31.9 $\pm$ 8.0  \\
%  \hline
%  J\&R sampling, valid loss and accuracy values & 63.0 & \textbf{39.1} $\pm$ 14.3  \\
%  \hline
%  Randomized J\&R valid loss and accuracy values & 25.0 & 18.9 $\pm$ 2.4 \\
%  \hline\hline
%  Topological features derived from grid sampling & 31.5 & 24.5 $\pm$ 4.3 \\
%  \hline
%  Topological features derived from naive sampling & 33.3 & 28.0 $\pm$ 5.6 \\
%  \hline
%  Topological features derived from J\&R sampling & \textbf{45.4} & \textbf{29.6} $\pm$ 7.2 \\
%  \hline
%  Randomized J\&R topological features & 20.4 & 14.9 $\pm$ 3.6 \\
% %  \hline \hline
% %  Best & & \\
%  \hline
% \end{tabular}
% \end{table}

% Across the sampling procedures, the loss and accuracy values collected with naive sampling achieve the greatest maximum accuracy on the 5 class generalization classification task, namely 66.7\%. The jump and retrain valid samples achieve slightly less at 63.0\% max accuracy but with a significantly better mean accuracy at 39.1\% than the other features. We remind the reader that the retrain and validation data sets are subsets of the original training data set, i.e. train set = retrain set $\cup$ valid set. The jump and retrain retrain data and grid sampling train data are the worse at predicting generalization with maximum accuracies of 45.4\% and 48.1\% respectively. In all cases the sampling seems to truly hold information about the network generalization capabilities since it performs significantly better than random and then the randomized J\&R features. These results seem to confirm our earlier hypothesis, that grid like sampling is not the most efficient way to sample the loss landscape if we wish to uncover links with the network's ability to generalize. The fact that we can look into multiple directions seem to benefit the naive sampling data.

% If we look at the topological features we see that the jump and retrain sampling allows for a better computing of the topological features of the loss landscape that are linked with generalization since. With a 45.4\% maximum accuracy it performs almost as well on the generalization classification task as the direct loss and accuracy data from the grid and J\&R retrain sampling procedures. While the mean of the accuracies is not very large for all features and the standard deviation can be pretty big, it is important to note that the 11 classifiers were not tuned to any of the features to not favor any of the sampling procedures.


% \subsection{Effect of network architecture and training hyperparameters}
% As mentionned in Section \ref{s:related_work}, \cite{im2016empirical_loss_surfaces} have found that for a given network and parameter initialization, different optimizers find different minima surrounded by regions of distinct geometrical characteristics. On the other hand, \cite{Goldstein_LL_NIPS2018_7875} found that the flatness of the region surrounding found minima varies with network depth and width. We go one step further than past experiments and ask: can we predict the depth, width of a network or the training hyperparameters with which the optimum was reached by looking at points sampled from the loss landscape and the topological features of the landscape? While we only consider the SGD optimization algorithm, we try to isolate the relationship between the loss landscape geometrical and topological features and either the batch size, weight decay or data augmentation. To our knowledge it is the first time that this has been done.

% To answer this question we use the same set up and classification task as presented in the previous subsection. Instead of trying to determine a network's generalization accuracy we try to determine it's depth, width or the hyperparameter values used for the training procedure with which the minimum was reached. For the complete list of values used for each considered parameters please refer to the first paragraph of Section \ref{ss:experimental setup}.

% \begin{table}
% \centering
% \caption{Maximum of the 11 classifiers accuracies (\%) on the depth, width, batch size, weight decay or data augmentation classification task with different features.}
% \label{tab:hparams}
%  \begin{tabular}{|M{4cm}|M{1.2cm}|M{1.2cm}|M{1.2cm}|M{1.2cm}|M{1.2cm}|}
%  \hline
%  Features & Depth & Width & Batch size & Weight decay & Data aug. \\
%  \hline
%  Theoretical random (1/\#classes)& 33.3 & 50.0 & 33.3 & 33.3 & 50.0\\
% \hline \hline
%  Grid, train loss and accuracy &\textbf{78.7}&80.6&38.9&64.8&96.3\\
%  \hline
%  Naive, train loss and accuracy &65.7&\textbf{83.3}&41.7&76.9&95.4\\
%  \hline
%  J\&R, retrain loss and accuracy & 54.6 & 78.7 & \textbf{50.0} & 85.2 & \textbf{97.2}\\
%  \hline
%  J\&R, valid loss and accuracy & 55.6 & 79.6 & \textbf{50.0} & \textbf{88.9} & \textbf{97.2}\\
%  \hline
%  Randomized J\&R valid loss and accuracy & 52.8 & 72.2 & 38.0 & 46.3 & 58.3 \\
%  \hline\hline
% Grid, topological features & 50.9 & \textbf{81.5} & 35.2 & 61.1 & 64.8 \\
%  \hline
%  Naive, topological features & \textbf{63.0} & 51.9 & \textbf{38.9} & \textbf{70.4} & 61.1 \\
%  \hline
%  J\&R, topological features & 54.6  & 72.2 & \textbf{
% 38.9} & 58.3 & \textbf{80.6} \\
%  \hline
%  Randomized J\&R topological features & 42.6 & 51.9 & \textbf{38.9} & 41.7 & 53.7 \\
% %  \hline \hline
% %  Best &33.3&50.0&33.3&33.3&50.0\\
%  \hline
% \end{tabular}
% \end{table}

% Version with mean and standard deviation (doesn't fit in page)

% \begin{table}
% \label{tab:hparams}
% \centering
% \caption{Maximum of the 11 classifiers accuracies (\%) on the depth, width, batch size, weight decay or data augmentation classification task with different features.}
%  \begin{tabular}{|M{4cm}|M{0.5cm}|M{1cm}|M{0.5cm}|M{1cm}|M{0.5cm}|M{1cm}|M{0.5cm}|M{1cm}|M{0.5cm}|M{1cm}|}
%  \hline
%  Features & \multicolumn{2}{c|}{Depth} & \multicolumn{2}{c|}{Width} & \multicolumn{2}{c|}{Batch size} & \multicolumn{2}{c|}{Weight decay} & \multicolumn{2}{c|}{Data aug.} \\
%  \hline
%  Theoretical random (1/\#classes)& 33.3& 30.0$\pm$3.0 & 50.0&  & 33.3&  & 33.3&  & 50.0& \\
% \hline \hline
%  Grid, train loss and accuracy &\textbf{78.7}& &80.6& &38.9& &64.8& &96.3& \\
%  \hline
%  Naive, train loss and accuracy &65.7& &\textbf{83.3}& &41.7& &76.9& &95.4& \\
%  \hline
%  J\&R, retrain loss and accuracy & 54.6&  & 78.7&  & \textbf{50.0}&  & 85.2&  & \textbf{97.2}& \\
%  \hline
%  J\&R, valid loss and accuracy & 55.6&  & 79.6&  & \textbf{50.0}&  & \textbf{88.9}&  & \textbf{97.2}& \\
%  \hline
%  Randomized J\&R valid loss and accuracy & &  & &  & &  & &  & &  \\
%  \hline\hline
% Grid, topological features & &  & &  & &  & &  & &  \\
%  \hline
%  Naive, topological features & &  & &  & &  & &  &  & \\
%  \hline
%  J\&R, topological features & &  & &  & &  & &  & &  \\
%  \hline
%  Randomized J\&R topological features & &  & &  & &  & &  & &  \\
%  \hline \hline
%  Best &33.3& &50.0& &33.3& &33.3& &50.0& \\
%  \hline
% \end{tabular}
% \end{table}

% If we look solely at the loss and accuracy samples we observe that there is already significant predictive information stored inside the sampled data. The grid sampled data achieves the best classification accuracy for the depth of the networks, namely 78.7\% while random is 33.3\%. This is consistent with the results of \cite{Goldstein_LL_NIPS2018_7875} which have used their linear interpolation (grid-like) loss landscape visualization technique to show that the flatness of the loss region surrounding the optimum significantly varies with network depth. The naive loss and accuracy sampled are the most predictive of width with 83.3\% classification accuracy. For batch size weight decay and data augmentation the jump and retrain sampling method seems the most informative. An interesting result is the 88.9\% maximum classification accuracy for weight decay while the random is only 33.3\%. It seems that the weight decay value used during training to reach an optimum has significant impact on the characteristics of the region surrounding that optimum. Additionally, the jump and retrain sampling procedure seems to be able to extract these characteristics pretty efficiently and better than the other sampling methods. Another interesting result is the very high accuracy reached by all features when predicting if data augmentation was used or not. This is consistent with prior belief from the literature that data augmentations forces the optimizer into wider regions since the optimum must accommodate a more complex set of training examples.

% The topological features perform particularly well on the width classification task with the ones derived from grid sampling reaching 81.5\% maximum accuracy. They also seem to hold significant information about network depth, weight decay and data augmentation since they perform significantly better than random and than the randomized features. It is only for on batch-size classification task that the topological features seem to not perform much better than the randomized features.

% \subsection{Ablation study}
% % The topological features presented in tables \ref{tab:generalization} and \ref{tab:hparams} were computed using a kNN connectivity matrix based on the cosine distance PHATE diffusion potentials and 25 by 25 persistence images.
% In order to properly evaluate the effectiveness of our analysis pipeline we ran an ablation study by computing the topological features using kNN connectivity matrices, with $k\in\{5,10,15,20\}$, based on the euclidean and cosine distance matrices between the sampled points in parameter space as well as on the PHATE euclidean or cosine diffusion potentials. For each of these connectivity matrices we computed the loss-level filtration persistence diagrams and considered multiple representations of these diagrams, namely persistence images with size $n$ by $n$ for $n\in\{10, 25, 100\}$.


==> obsolete files/robustness.tex <==
\vspace{-2mm}
\subsection{Robustness}\label{ss:robustness}

\vspace{-2mm}
One of the main problems encountered in previous attempts to visualize ANN loss landscapes resides in the difficulty of comparing them across tasks and initializations. Here, we show that our visualization approach, applied to the results of jump-and-retrain experiments, alleviates this concern. To this end, we trained multiple WResNet28-2 networks by following the procedure described in Sec.~\ref{fig:generalization}, and starting from multiple parameter initializations. For each initialization, we found one good (\textasciitilde94\% test acc.) and one bad optima (\textasciitilde86\% test acc.), giving the jump-and-retrain results shown in Fig.~\ref{fig:robustness}. Further, we also trained a similar network on the CIFAR100 dataset, following the same training procedure, except here the data augmentation was comprised not only of random horizontal flips and crops, but also of random rotations of up to 45$^\circ$ in each direction and random modifications to the brightness, contrast, saturation and hue of the images. Since CIFAR100 poses a significantly harder classification task than CIFAR10, our networks only reaches \textasciitilde60\% test accuracy for the bad optimum trained without data augmentation and weight decay, and \textasciitilde70\% test accuracy for the good optimum. The fact that the networks only reached 70\% accuracy is just a reflection of the complexity of the task, with better accuracy requiring a better fine-tuning of the architecture and the training procedure. The results of these experiments are shown in Fig.~\ref{fig:robustness}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/robustness_figure.png}
    \caption{2D PHATE embeddings of the jump and retrain experiment ran on different initialization for the WResNet28-2 network on CIFAR10 (\textbf{a,b,c and d}) and on CIFAR 100 (\textbf{e and f}), colored by epoch of retraining. Patterns that resemble bad generalization are exhibited in the first plot for all three settings as in (a), (c) and (e), while good generalization patterns are shown in the second plots (b), (d) and (f). It demonstrates that our approach is robust across tasks. See Appendix \ref{a:robustness_hi_res} for a higher resolution version.}
    \label{fig:robustness}
    \vspace{-0.1 in}
\end{figure}

The plots for different initializations of the WResNet28-2 are consistently showing the same star-shaped patterns, characterizing the retraining trajectories surrounding minima that generalize well. The plots for the bad minima also share a similar pattern, not only across initialization but also across tasks. Strikingly, the star-shaped pattern is even better defined in Fig.~\ref{fig:robustness}f, corresponding to the good optimum of WResNet28-2 trained on CIFAR100. This offers a key insight into the effect of regularization on the geometric characteristics of the found minima. It seems that regularization techniques enhance generalization by forcing the optimizer into wider valleys.

==> obsolete files/s_memorization.tex <==
\subsection{Memorization}\label{ss:memorization}
Recent papers \citep{Zhang2017UnderstandingDL, closer_look_memorization, dnns_don't_learn_via_mem} have established the ability of neural networks to completely memorize the data set through variations of the random label experiment. These papers have put forward this ability, neural networks have a natural tendency to generalize and to learn general rules and patterns in the data before memorizing datum level details.

As mentioned earlier however, the fact that neural nets settle into a generalization optima rather than a memorization one is a direct consequence of the training process, which is itself highly dependent on the loss-landscape of the network. This raises the following question: what are the geometric characteristics of the loss-landscape which allow optimizers to reach good generalization optima? Also, are there significant geometric differences between the regions surrounding each type of optima?

The WResNet28-2 trained on CIFAR10 achieved \textasciitilde0 loss (\textasciitilde100\% accuracy) on the training set regardless of whether we train for generalization in standard ways or for memorization using random labels. From past work and earlier discussion we know that when the models generalize well, the loss-landscape tends to be flat. How will the regions surrounding each type of optima compare?

%\subsubsection{Experiments}
%The same "jump and retrain" experiment presented in Section \ref{ss:generalization} was used here except one of the optimum used was achieved not with the standard CIFAR10 training set but with a scrambled labels version of it. The network was able to completely memorize the data as it achieved 100\% accuracy. The two networks trained for generalization had also achieved 100\% accuracy but on the unmodified CIFAR10 training data.
%\subsubsection{Results}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/memorization_figure.png}
    \caption{2D PHATE embeddings computed with cosine distance of the jump and retrain experiment conducted on one good and one bad generalization optima which achieved 94.39\% and 87.29\% accuracy on the test data respectively as well as on one memorization optimum. The three networks achieved 100\% accuracy on the training data and all the plots are colored according to the accuracy on the retraining data at each point in parameter space.}
    \label{fig:optim_compare}
\end{figure}

It seems like the distinct, star-like pattern, is specific to the trajectories surrounding optima that generalize well. The memorization optimum, despite not having the same pattern, shows one key characteristic: the retraining trajectories seem to reach optimal loss on the training data a lot quicker during the retraining. When compared to the bad generalization optimum, the memorization also looks "flatter" since the trajectories converge more directly towards the middle of the plot and no trajectories seem to get stuck towards the borders of the visualizations.

We recognize the possibility that the "sharpness" of memorization optima might not be directly comparable to that of generalization optima since, by scrambling the labels of the training set, we effectively change the task and the structure of the data in a significant way.

==> obsolete files/s_proposed_visualization.tex <==
\section{Proposed visualization method}
In this paper we propose a novel method for visualizing ANN loss-landscapes. It utilizes the modern dimensionality reduction technique PHATE (\cite{phate}) which was shown to preserve high-dimensional non-linear patterns in data better than similar methods. In particular, PHATE excels at visualizing trajectory patterns in high dimensional space, which helps visualize the evolution of the high-dimensional network weights. 

The loss landscape is a complex object which, for most modern ANNs, lives in Euclidean spaces with more than a million dimensions (one for each trainable weight).  We argue that visualizations of the loss landscape must help inform us about practical characteristics of our models: how well do our models learn and how well will they be able to generalize? Can we know if one trained network will perform better than another on the test data without employing additional test data? Can we properly visualize multiple training trajectories in a manner that makes relevant comparisons possible? To answer most of these questions it is of little use to visualize parts of the loss landscape that would have been ignored by the network optimizer.

To our knowledge, our method is the first non-linear loss-landscape visualization method and the first to aggregate multiple possible trajectories of network optimizers in order to plot an evocative view of what really happens in this high dimensional space despite the low dimensionality of the final embedding.

\subsection{Why PHATE?}
PHATE excels at finding trajectory and branches-like patterns in data. Other state of the art dimensionality reduction or visualization methods such as t-SNE \citep{tsne} and UMAP \citep{umap} were designed to reveal manifold like structure in large data sets of high-dimension. Such algorithms are less adapted to reveal trajectories structures since they tend to locally group data points that are close in the high-dimensional latent space. Figure \ref{fig:dim_red_comparison} shows a comparison of the dimensionality reduction methods mentioned and how they embed, in 2D space, the training trajectories of a WResNet28-2 model (wide ResNet \citep{wide_resnet} of depth 28 and 2 times as wide as a standard ResNet \citep{resnet}) on the CIFAR10 dataset \citep{cifar10}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/dim_red_comparison_cos-dist_45-size_dots.png}
    \caption{Low-dimensional embeddings obtained through different dimensionality reduction algorithms with cosine distance of WResNet28-2 parameters saved at each point during training on the CIFAR10 data set. 20 training trajectories are plotted, each starting after taking a step of size $\in \{0.25, 0.5, 0.75, 1\}$ in one of 5 normalized random directions from a known optimum for the task and model considered. See Section \ref{ss:generalization} for more details on the origin of the data.}
    \label{fig:dim_red_comparison}
\end{figure}

The network weights in Fig\ref{fig:dim_red_comparison} were collected from training with 20 random initializations that are combinations of 5 directions and 4 step sizes stemming from a known optimum. As expected, t-SNE and UMAP arrange in cluster points corresponding to similar training trajectories since such points are close in parameter space. Although some path-like structure is visible inside each cluster it is virtually impossible to compare trajectories since the global structure of the data and how the trajectories are linked to one another were lost. The simple linear dimensionality reduction method PCA captures some of the global structure of the data since the trajectories are aligned according to the direction leaving the optimum, with training trajectories corresponding to smaller step sizes placed more towards the center. However, PCA does this because the largest amount of variability in the data is caused by the structure of the experiment, namely the random directions and the step sizes. Little to no variability from the actual training trajectories is captured in the low-dimensional embedding. PHATE captures more intra-trajectory variability while maintaining the global structure of the data. The initial points corresponding to the same direction leaving the optimum are clustered together since the metric used is cosine distance. This allows the reader to 


==> obsolete files/z1_vgg.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/robustness_figure.png}
    \caption{2D PHATE embeddings of the jump and retrain experiment ran on different initialization for the WResNet28-2 network (a, b, c, d), on VGG9 trained on CIFAR10 and on a 16x16 MLP trained on MNIST.}
    \label{fig:vgg}
\end{figure}

The plots for different initializations of the WResNet28-2 are consistently showing the same patterns. While the VGG9 and MLP plots do not resemble the WResNet28-2 ones they are consistent with the results of \cite{Goldstein_LL_NIPS2018_7875} which has found that skip connections have a smoothing effect on the loss-landscape and that VGG9-like networks tend to have sharper optima, surrounded by significant non-convexities, as opposed to the flatter optima of ResNet models with comparable generalization capabilities.


\textcolor{red}{The initial goal of this section was to show that the method can be used to compare across initializations, tasks and network architecture. The data I have so far doesn't really support this.}

==> sections/name.tex <==
\vspace{-13pt}
\section{Discussion and conclusion}
\vspace{-12pt}
We propose a novel approach to dynamically sample the loss landscapes of deep learning models which takes theoretical inspiration from the fields of Riemannian geometry and dynamical systems. Our sampling method efficiently samples points form the low-loss manifolds surrounding minima found through gradient descent. The resulting sampled data holds more information than past loss landscape sampling methods about the geometry of the loss landscape, the network ability to generalize at the optimum and the training procedure and regularization used to reach that optimum. We then present a new loss landscape visualization method based on the state-of-the-art PHATE dimensionality reduction method, which is able to reconstruct the high-dimensional trajectories sampled in two dimensional representations. Our approach enables geometric exploration of the sampled manifolds and regions surrounding generalization and memorization optima, found via ANN training, to provide insight into generalization capabilities and training of the network. Finally, topological data analysis enables us to characterize these regions through the computation of their topological features. We found that weight decay, a powerful regularization technique, allows ANN optimizers to find minima in regions of lower topological activity. An interesting research direction would be to try to apply dimensionality reduction techniques that better take into account the time dependency of the data. We expect in future work our sampling, visualization and topological characterization approaches to enable more methodical paradigms for the development of ANNs that generalize better, train faster, and to provide fundamental understanding of their capabilities.



==> sections/related_work.tex <==
\vspace{-5pt}
\section{Related work}\label{s:related_work}
\vspace{-7pt}
\subsection{Loss landscape visualization}\label{ss:ll_visualization}
%
Loss landscape visualization methods have been proposed in numerous contexts. \citet{goodfellow2014qualitatively} proposed the ``linear path experiment'' where the loss of an ANN is evaluated at a series of points $\theta=(1-\alpha)\theta_i + \alpha \theta_f$ for different values of $\alpha \in [0,1]$ and $\theta_i,\theta_f$ corresponding to the initial parameters of the model and the found optima in parameter space respectively. This one-dimensional linear interpolation method has allowed them to show that popular state of the art ANNs typically do not encounter significant obstacles along a straight path from initialization to convergent solution. They also used the method to visualize the loss along directions connecting two distinct minima and to show that these are linearly separated by a region of higher valued loss.

This method was further developed by \citet{im2016empirical_loss_surfaces}, who adapted it to enable the visualization of two-dimensional projections of the loss-landscape using barycentric and bilinear interpolation for groups of three or four points in parameter space. This analysis method has allowed them to establish that despite starting with the same parameter initialization, different optimization algorithms find different minima. Furthermore, they noticed that the loss-landscape around minima have characteristic shapes that are optimizer-specific and that batch-normalization smoothens the loss function.

More recently, \citet{Goldstein_LL_NIPS2018_7875} have addressed the \textit{scale invariance} and \textit{network symmetries} problems discussed in \citet{neyshabur2017exploring} and \citet{dinh2017sharp_minima_gen}, which prevented meaningful comparisons between loss-landscape plots from different networks. They proposed 1D and 2D linear interpolation plots, similar to past techniques, but where they used filter-wise normalized directions to remove the scaling effect. This method has allowed them to visualize and compare the regions on the loss-landscape surrounding minima coming from multiple networks in a meaningful way and to correlate the ``flatness'' of the region to the generalization capabilities of the corresponding network. Furthermore, they studied the effects of the network depth, width and the presence of skip connections on the geometry of the loss-landscape and on network generalization. %They also proposed using normalized PCA directions to plot training trajectories in two dimensions.

\subsection{Generalization and importance of studying the loss landscape}
Ensuring that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. The idea that a network's ability to generalize is linked to the geometry of the loss landscape around the optima was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers~\citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Following the underlying idea of these propositions, we believe that studying the geometry of the loss landscape around minima has the potential of uncovering key characteristics about the network's ability to generalize. 

Furthermore, the importance of loss landscape visualization methods like the one presented in this paper increases with the growing scientific community interest in furthering our understanding of ANNs. As our understanding of this landscape gets deeper, we start uncovering more and more high-dimensional and complex geometric and topological characteristics. For instance, \citet{essentially_no_barriers} have found nonlinear pathways in parameter space connecting distinct minima, along which the training and test errors remain small and losses are consistently low. This suggests that minima are not situated in isolated valleys but rather on connected manifolds representing low loss regions. However, such characteristics are intrinsically high-dimensional, making linear methods inadequate to visualize these structures. Even in standard applications of the linear methods one inevitably asks if the thousands (or even millions) of unseen directions do not hide critical features of the landscape, and if the visualized linear path is relevant to what happened during training.

\subsection{Manifold learning and topological data analysis}
In this paper, we suggest the use of modern manifold learning and topological data analysis techniques to study the complex loss landscape of ANNs. Manifold learning techniques have been extensively used in recent years to successfully study the internal learned representations of deep networks and highlight their complex geometric structures and intrinsic dimensionality \citep{gigante2019visualizing, horoi2020internal, recanatesi2018signatures, farrell2019dynamic, maheswaranathan2019universality}. Here we further advance theses lines of work to provide new applications and insights in the study of ANN optimization and generalization.

To our knowledge, this is the first time topological data analysis (TDA) has been applied to the study of ANN loss landscapes. 
However, the application of algebraic topology to the analysis of real-valued functions defined on manifolds is not novel, and is in fact at the heart of Morse theory, developed by Marston Morse and others during the 20$^{\text{th}}$ century~\citep{morse1925relations, milnor2016morse}. 
More recently, numerous efficient computational algorithms for solving concrete problems related to algebraic topology have been developed in the field of computational topology \citep{Edelsbrunner10}.
A particular problem that can be solved through the use of TDA algorithms is the topological characterization of critical points of real-valued functions defined on manifolds \citep{Gyulassy08, Gyulassy2006topological, bremer2004topological}. If the ambient dimension of the manifold is low~(2D or 3D), such a characterization gives rise to a decomposition of a function in terms of regions of similar gradient behavior~(the classical example is a function with two peaks defined on $\mathbf{R}^2$; here, there would be a decomposition into regions that measure which peak is ``closer''). This decomposition is known as the Morse--Smale complex. 
The Morse--Smale complex can be computed from the critical points of the respective function and its unstable manifolds as defined by the dynamics of gradient descent~(or ascent). 
The hierarchical structure of the complexes and the function's topological features are found by considering the succession of critical points and unstable manifolds in the increasing sequence of the function's sublevel sets, i.e., the set of all points on the manifold whose function value is less than or equal to a pre-defined threshold. 
%
The difference between the function values of different critical points---equivalently, this is the difference between the ``appearance'' and ``disappearance'' of a topological feautre---is referred to as the \emph{persistence}. Persistence  can be used to simplify a given function by smoothing out features; this is typically achieved by cancelling related pairs of critical points whose persistence fails to satisfy a certain simplification threshold.
Such analysis methods have been successfully applied in the field of electrochemistry, for instance, to characterize the topology of energy landscapes of different molecules \citep{Gyulassy2006topological, bremer2004topological}. 
This directly relates to our work since the loss-landscape associates a loss value to each point in the parameter space of the ANN and we wish to characterize the topology of this landscape. The primary difference to existing work is that we are dealing with a manifold whose~(ambient) dimension is much higher, thus precluding the analytical calculation of the Morse--Smale complex.

%
% \subsection{Generalization and sharpness of the landscape at the optimum}
% Making sure that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. It is so important that oftentimes large fractions of the scarcely available data are not used for training but rather for testing, to ensure that models indeed learn to solve the task in a relevant manner without overfitting their training data. Arguably one of the most important and general questions in machine learning at the moment is: by looking only at a given trained model and its training data, can we predict how well the model will perform on unseen data? There was even an entire NeurIPS 2020 competition entirely focused on answering this question \citep{pgdl_neurips2020}. 
%
% Previous work offers a partial and vague answer to this question by linking the ``flatness'' of neural network optima to the extent to which the network is able to generalize. This idea was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers \citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Following the underlying idea of these propositions, we believe that studying the geometry of the loss landscape around minima has the potential of uncovering key characteristics about the network's ability to generalize.

% \subsection{Importance of studying the loss landscape}
% In this paper, we suggest the use of modern manifold learning and topological data analysis techniques to study the complex loss-landscape of ANNs. Manifold learning techniques have been extensively used in recent years to successfully study the internal learned representations of deep networks and highlight their complex geometric structures and intrinsic dimensionality \citep{gigante2019visualizing, horoi2020internal, recanatesi2018signatures, farrell2019dynamic, maheswaranathan2019universality}. TDA on the other hand has recently been applied to analyze brain imaging data \citet{rieck2020_fmri_cubical} and has been gaining popularity in the field of deep learning \citet{}. Here we further advance theses lines of work to provide new applications and insights in the study of ANN optimization and generalization.

==> sections/related_work_short.tex <==
\vspace{-7pt}
\section{Related work}\label{s:related_work}
\vspace{-10pt}
% \subsection{Loss landscape visualization}\label{ss:ll_visualization}
%
Loss landscape visualization methods have been proposed in numerous contexts. \citet{goodfellow2014qualitatively} proposed the ``linear path experiment'' where the loss of an ANN is evaluated at a series of points $\theta=(1-\alpha)\theta_i + \alpha \theta_f$ for different values of $\alpha \in [0,1]$ and $\theta_i,\theta_f$ corresponding to the initialization and optimum respectively. This one-dimensional linear interpolation method has allowed them to show that popular state of the art ANNs typically do not encounter obstacles along a straight path from initialization to convergent solution and that distinct minima are linearly separated by a region of higher valued loss. This method was further developed by \cite{im2016empirical_loss_surfaces}, who adapted it to enable the visualization of two-dimensional projections of the loss-landscape. This analysis method has allowed them to establish that despite starting with the same parameter initialization, different optimization algorithms find different minima surrounded by regions of characteristic shapes that are optimizer-specific. More recently, \citet{Goldstein_LL_NIPS2018_7875} have addressed the \textit{scale invariance} \citep{neyshabur2017exploring} and \textit{network symmetries} \citep{dinh2017sharp_minima_gen} problems  which prevented meaningful comparisons between loss-landscape plots from different networks. They proposed 1D and 2D linear interpolation plots where they used filter-wise normalized directions to remove the scaling effect. This allowed them to visualize and compare the regions on the loss-landscape surrounding minima coming from multiple networks.
%in a meaningful way. 
% and to correlate the ``flatness'' of the region to the generalization capabilities of the corresponding network.% Furthermore, they studied the effects of the network depth, width and the presence of skip connections on the geometry of the loss-landscape and on network generalization. %They also proposed using normalized PCA directions to plot training trajectories in two dimensions.

% Ensuring that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. The idea that a network's ability to generalize is linked to the geometry of the loss landscape around the optima was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers \citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Following the underlying idea of these propositions, we believe that studying the geometry of the loss landscape around minima has the potential of uncovering key characteristics about the network's ability to generalize. 

% Furthermore, the importance of loss landscape visualization methods like the one presented in this paper increases with the growing scientific community interest in furthering our understanding of ANNs. As our understanding of this landscape gets deeper, we start uncovering more and more high-dimensional and complex geometric and topological characteristics. For instance, \citet{essentially_no_barriers} have found nonlinear pathways in parameter space connecting distinct minima, along which the training and test errors remain small and losses are consistently low. This suggests that minima are not situated in isolated valleys but rather on connected manifolds representing low loss regions. However, such characteristics are intrinsically high-dimensional, making linear methods inadequate to visualize these structures. Even in standard applications of the linear methods one inevitably asks if the thousands (or even millions) of unseen directions do not hide critical features of the landscape, and if the visualized linear path is relevant to what happened during training.

% In this paper, we suggest the use of modern manifold learning and topological data analysis techniques to study the complex loss landscape of ANNs. Manifold learning techniques have been extensively used in recent years to successfully study the internal learned representations of deep networks and highlight their complex geometric structures and intrinsic dimensionality \citep{gigante2019visualizing, horoi2020internal, recanatesi2018signatures, farrell2019dynamic, maheswaranathan2019universality}. Here we further advance theses lines of work to provide new applications and insights in the study of ANN optimization and generalization.

%
% \subsection{Generalization and sharpness of the landscape at the optimum}
% Making sure that machine learning models can generalize to new data is one of the most important steps in solving any data analysis task, and is a core problem in the field. It is so important that oftentimes large fractions of the scarcely available data are not used for training but rather for testing, to ensure that models indeed learn to solve the task in a relevant manner without overfitting their training data. Arguably one of the most important and general questions in machine learning at the moment is: by looking only at a given trained model and its training data, can we predict how well the model will perform on unseen data? There was even an entire NeurIPS 2020 competition entirely focused on answering this question \citep{pgdl_neurips2020}. 
%
% Previous work offers a partial and vague answer to this question by linking the ``flatness'' of neural network optima to the extent to which the network is able to generalize. This idea was initially presented in \citet{Hochreiter1997_flat_minima} and has recently been the focus of numerous papers \citep[e.g.,][]{entropy_sgd,keskar2016large_batch,swirszcz2016local_minima,dinh2017sharp_minima_gen,Goldstein_LL_NIPS2018_7875}. Flat minima in parameter space, around which the value of the loss function is fairly constant, are believed to correspond to configurations where the network generalizes well to the unseen data. Sharp minima, on the other hand, correspond to ones where the network is expected to generalize poorly. Following the underlying idea of these propositions, we believe that studying the geometry of the loss landscape around minima has the potential of uncovering key characteristics about the network's ability to generalize.

% \subsection{Importance of studying the loss landscape}

% In this paper, we suggest the use of modern manifold learning and topological data analysis techniques to study the complex loss-landscape of ANNs. Manifold learning techniques have been extensively used in recent years to successfully study the internal learned representations of deep networks and highlight their complex geometric structures and intrinsic dimensionality \citep{gigante2019visualizing, horoi2020internal, recanatesi2018signatures, farrell2019dynamic, maheswaranathan2019universality}. TDA on the other hand has recently been applied to analyze brain imaging data \citet{rieck2020_fmri_cubical} and has been gaining popularity in the field of deep learning \citet{}. Here we further advance theses lines of work to provide new applications and insights in the study of ANN optimization and generalization.
